DISTWAR: Fast Differentiable Rendering on Raster-based Rendering Pipelines

Differentiable rendering is a technique used in an important emerging class of visual computing applications that involves representing a 3D scene as a model that is trained from 2D images using gradient descent. Recent works (e.g. 3D Gaussian Splatting) use a rasterization pipeline to enable rendering high quality photo-realistic imagery at high speeds from these learned 3D models. These methods have been demonstrated to be very promising, providing state-of-art quality for many important tasks. However, training a model to represent a scene is still a time-consuming task even when using powerful GPUs. In this work, we observe that the gradient computation phase during training is a significant bottleneck on GPUs due to the large number of atomic operations that need to be processed. These atomic operations overwhelm atomic units in the L2 partitions causing stalls. To address this challenge, we leverage the observations that during the gradient computation: (1) for most warps, all threads atomically update the same memory locations; and (2) warps generate varying amounts of atomic traffic (since some threads may be inactive). We propose DISTWAR, a software-approach to accelerate atomic operations based on two key ideas: First, we enable warp-level reduction of threads at the SM sub-cores using registers to leverage the locality in intra-warp atomic updates. Second, we distribute the atomic computation between the warp-level reduction at the SM and the L2 atomic units to increase the throughput of atomic computation. Warps with many threads performing atomic updates to the same memory locations are scheduled at the SM, and the rest using L2 atomic units. We implement DISTWAR using existing warp-level primitives. We evaluate DISTWAR on widely used raster-based differentiable rendering workloads. We demonstrate significant speedups of 2.44x on average (up to 5.7x).

==> text_srcs2/abstract_test.tex <==

\begin{itemize}
    \item Differential rendering is an important and emergent class of workload
    \item These applicaiont
\end{itemize}




==> text_srcs2/background.tex <==
\noindent 

\subsection{Learning Scene Representations with Differentiable Rendering}

In several tasks such as 3D scene reconstruction and inverse rendering, the training pipelines typically involves producing an image from a parameterized scene representation, and comparing this with a ground truth image (as shown in Fig.~\ref{fig:inverse_rendering}). A loss function which measures the difference between the ground truth image and the rendered image is then computed.
This loss function is minimized by backpropagating the loss derivative to obtain the derivative with respect to the scene parameters, and then applying gradient descent on these parameters.
In order to do this, a differentiable renderer, which computes the loss derivative with respect to scene parameters is used.


\todo{explain with circled numbers}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/inv_render_intro.pdf}
    \caption{Common differentiable rendering optimization pipeline.}
    \label{fig:inverse_rendering}
\end{figure}


\subsection{Rasterization based Rendering Pipeline}
\label{sec:bckg_diffrendering}
Traditional raster-based rendering pipelines (shown in Fig.~\ref{fig:rast_and_shading}) considers the scene being comprised of several fundamental geometric objects, or "primitives", in 3D space (such as a mesh composed of triangles, point cloud, spheres, etc.). These primitives are associated with rendering parameters (color/normal/material). These primitives are rendered as seen by a camera on screen using the rendering pipeline, consists of the pre-processing stage (primitive culling), rasterization, shading, and blending. The rasterizing and shading stages are described below: 1) \textbf{rasterization}: involves finding the list of primitives that are going to affect each pixel (known as \emph{fragments}) of the rendered image, and 2) \textbf{shading}: involves determining the color of each fragment that is going to contribute to the color of each pixel in the rendered image.

\textbf{Differentiable Rendering on rasterization pipeline}
\emph{Differentiable} raster-based rendering pipeline adds a backward pass routine which performs the sequence of steps depicted in Fig.~\ref{fig:backward_pass_renderer}. The routine receives as input a pixel-wise list of fragments (primitives which influence it's color) and loss gradient with respect to the fragment. 
This loss gradient with respect to the image is a large $H\times W\times C$ array, where $H, W, C$ correspond to the height, width (in number of pixels) and number of color channels of the image. Each element is the loss gradient with respect to the corresponding pixel's color channel. From each of these elements, it first computes the pixel's contribution of loss gradient w.r.t parameters of each primitive (corresponds to each fragment). It then aggregates these gradient contributions of all pixels for each primitive to produce the parameter gradient.
% Out of these stages, a vast amount of work in computer graphics literature over the years focused on optimizing the rasterization stage SW and shading stage~\cite{opengl}. The 

\begin{figure}[!htb]
    
    \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=0.85\linewidth, trim={5 0 0 0},clip]{figs/resterization_pipeline.pdf}
    \caption{Traditional rasterization based rendering pipeline}
    \label{fig:rast_and_shading}
    \end{subfigure}

    \begin{subfigure}{0.5\textwidth}
    \vspace{10pt}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/resterization_pipeline_bwd.pdf}
    \caption{Backward pass of the raster-based rendering pipeline}
    \label{fig:backward_pass_renderer}
    \end{subfigure}

    \caption{Forward and backward pass of the differentiable rendering pipeline}
\end{figure}

\subsection{GPU Architecture and Atomic Operations}
\label{sec:bckg_atomicprocessing}
% Each programmed as a set of SIMD instructions, known as a warp intructions that produce L2 
Fig.~\ref{fig:sm_baseline} depicts a streaming multiprocessor (SM) in a modern GPU that comprises multiple sub-cores \circled{1} (typically 4) and a memory I/O (MIO) block \circled{2} that handles memory transactions. Each sub-core consists of a register file, the frontend \circled{4} (instruction cache,  warp scheduler, instruction decoding and operand collection logic), execution units \circled{5}, and the load store (LDST) units \circled{6}. The MIO block consists of the L1 data cache, shared memory space and the load-store unit (LSU)\circled{3}.

Atomic instructions dispatched by the frontend \circled{4} are received at the LDST unit of the sub-core\circled{4}. The LDST unit produces a memory transaction for atomic request called by each active threads in the warp, and enqueues them to the instruction queue to the LSU unit in the MIO block \circled{3}. The LSU unit receives these request and issues them to the memory partition where the atomic requests are processed. The memory partition interfaces the L2 and global memory, and consists of render operation units (ROP)\circled{7}. These ROP units consist of floating point hardware that atomically computation and writes updates the atomic request's address to L2.  


\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{figs/bckg_gpu.drawio.pdf}
    \caption{Baseline model of a single GPU's SM Architecure}
    \label{fig:sm_baseline}
\end{figure}






% \subsubsection{GPU Memory consistency model in relation to atomic operations processing}

% The PTX instruction set, an intermediate representation instruction set used in NVIDIA GPUs, provides well defined semantics to express the memory consistency model, specified by the instruction set documentation~\cite{ptxisa, formalptxmc}. Most GPUs implement a version of Heterogeneous race-free for sequential consistency (HRF-for-SC) model. This model defines memory consistency across various scopes of memory, specifying memory ordering constraints for different memory regions visible to the programmer. Local and global scope~\cite{}. In this work, we are concerned with the accesses made by the memory mode ltowards the global scope This model provides semantics  by a store-release
% Shared weight parameters of the thread can be made via  memory operations 

% GPU memory consistency models is defined at scopes, for . The consistency model for \texttt{atom} and \texttt{red} instructions  is specified by 


% The memory consitency model provideds Load-acquire and store-release semantics


% The atomic operations of the GPU are processed at the memory partition which indexes a sereies of the L2 cache.  




==> text_srcs2/background3.tex <==





\subsection{GPU Baseline Architecture}
The baseline GPU architecture is shown in Fig.~\ref{fig:gpu_baseline}, which is representative of a modern GPU Streaming multiprocessor (SM) architecture~\cite{voltaarch}. Each SM consists of multiple (typically 4) sub-cores, or sub-partitions. Each sub-partition consists of it's own warp scheduler, register file, execution units.
The SM sends local, global and atomic memory requests from each sub-core are issued through the L1 instruction queue ~\cite{nsight_prof}. Atomic operations scheduled to this queue get get issued to the to memory subpartition. The memory partition constists of compute hardware (known as ROP units) which process the atomic request computation.

A high number of atomic requests made at the sub-core would lead to contention in the ROP units at the memory subpartition on processing of atomic requests. This causes contention in issuing of atomic instructions to the L1 instruction queues by each sub-core.


\begin{figure}[!htb]
    \centering
    % \includegraphics[width=0.75\linewidth]{figs/gpu_baseline.png}
    \includegraphics[width=0.75\linewidth]{figs/figure3(1).pdf}
    \caption{GPU baseline architecture.}
    \label{fig:gpu_baseline}
\end{figure}




% \subsection{Parametric Scene Representation and Differentiable Rendering}
\subsection{Differentiable Rendering}
Visual information of 3D space, such as positions/orientations of various objects, geometries of various shapes, color, etc can be analytically encoded with real numbers, or \emph{parameters}. This encoding of visual using parameters, or \emph{parameterized scene representations} allows computer graphics algorithms to process, render/display, transform or generate 3D visual  information by manipulating the parameters encoding the scene. 
Thus, these parameterized scene representations serve as a \emph{model} for 3D visual information of the scene, with the model's \emph{parameters} being the same as the scene parameters.

Differentiable rendering is a useful tool that enables applications to leverage machine learning techniques by treating the parameterized scene as a model whose parameters are to be \emph{learnt}. 
It allows for applying a standard tool from machine learning, namely \emph{gradient based optimization} for learning model parameters, described below. 


We describe here a classic and important problem in computer graphics: 3D scene reconstruction. 
3D scene reconstruction has several important applications in novel view synthesis, 3D scanning and modelling and photogrammetry. It involves learning scene parameters that encode the scene's information from a set of ground truth images to demonstrate the application of differentiable rendering.
The standard approach in applying machine learning methods to this problem is depicted in Fig.~\ref{fig:ml_diffrendering}. Starting from a parameterized scene, or "model" \circled{1},  a differentiable renderer can produce an image of this scene in its \emph{forward pass}\circled{2}. The degree of difference between the rendered image and a desired/reference image (known as a \emph{loss}) \circled{3} can be obtained by subtracting the RGB values of each pixels between rendered, and summing up these components. Machine learning methods apply gradient based optimization in minimizing this difference to find these scene parameters. 
This minimization is performed using gradient descent, which involves iteratively updating each model parameter by adding a small gradient of the loss function with respect to itself~\cite{gradient_descent}\todo{citation required?}.
A differentiable renderer is used to obtain the gradients of these models (3D scene representations), in the \emph{backward pass} \circled{4}. 


\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/inv_render_intro.pdf}
    \caption{Common differentiable rendering optimization pipeline.}
    \label{fig:ml_diffrendering}
\end{figure}



\subsection{Differentiable Rendering for Rasterization Pipelines}

A simple, yet effective model for encoding 3D visual information is to consider each object in the scene as being composed of several discrete geometric elements, or \emph{primitives}, in space. Each of these elements is associated with color information, and a position in space. 
This model of scene representation can be rendered  as follows:

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/inv_render_intro.pdf}
    \caption{Common differentiable rendering optimization pipeline.}
    \label{fig:primitive}
\end{figure}

A recent work in differentiable rendering, known as 3D gaussian splatting~\cite{3dgs}, models the scene with 3-dimensional gaussians as the geometric primitives.
Fig.~\ref{fig:primitive} represents the primitive with an ellipsoids.
Under this framework, the \emph{model} is simply a set of these ellipsoids in space. The model's parameters are the parameters associated with each of the ellipsoids (which are it's position of it's centroid, orientation and color information) \circled{1}. For reconstruction problems, the \emph{forward pass} involves rendering using rasterization pipeline into an image. \circled{2}.  The \emph{backward pass} \circled{3} involves computing the gradient of the loss.




% Raster based graphics methods are a special class of rendering. These methods express the visual information of the scene with a set of primitives - a geometric object in 3D space








==> text_srcs2/conclusion_test.tex <==

We introduce \projname, the first work



==> text_srcs2/evaluation2.tex <==
We evaluate \projname on several configurations, which we describe in Table~\ref{tab:methodconfigurations}. \texttt{\projname-SW-B-X} and \texttt{\projname-SW-S-X} implement \projname-SW that use butterfly reduction and serialized addition to do reduction respectively, with $X$ set as the balancing hyperparameter. 
\texttt{cccl} is on using the NVIDIA CCCL library~\cite{cccl, cub} library to do the warp-level reduction for each atomic reduction, on checking if all threads update the same parameter.
% \texttt{\projname-SW-B} and \texttt{\projname-SW-S} represent \projname-SW mechanisim on using the best-tuned balancing threshold for each corresponding workload. 
\texttt{\projname-HW} represents our hardware implementation \projname-HW.
with how on how our approach performs on buffering atomic requests \texttt{AB} representative of the work described in local atomic buffering, atomic requests in L1/shared memory cache~\cite{lab}. \todo{fix}

\begin{table}[h!]
 \centering
  \caption{Evaluation Configurations}
  \label{tab:methodconfigurations}
  \begin{tabular}{|l|l|}
    \hline
     \textbf{Configuration}    & \textbf{Description} \\
    \hline
    \multirow{2}{*}{\texttt{\projname-SW-B-X}} &  SW approach with butterfly-reduction, \\                                      & with X as the balance threshold   \\
    \hline
    \multirow{2}{*}{\texttt{\projname-SW-S-X}} &  SW approach with serialized-reduction, \\                                      & with X as the balance threshold   \\

    \hline
    \texttt{CCCL} &  CCCL~\cite{cccl} warp reduction library on each primitive \\     

    \hline
    \texttt{\projname-HW} &  \projname HW implementation    \\             
    \hline
    \texttt{AB} &   Atomic Buffering at L1D level    \\             

    \hline

  \end{tabular}
\end{table}



\subsection{Speedup in SW}
Fig.~\ref{fig:end_to_end_speedup} shows the end-to-end speedup obtained on using \projname-SW (\texttt{\projname-SW-B} and \texttt{\projname-SW-S} implementations), for different values of balancing threshold parameter $X$ over baseline, on different HW platforms. 
We observe that \texttt{\projname-SW-B} and \texttt{\projname-SW-S} are able to provide a speedup of up to $3.40\times$ and $\times$, and on average $1.4\times$ and $\times$ on an RTX 4090 and an RTX 3060 GPU respectively. 

% \begin{figure}[!htb]
% \begin{subfigure}{0.49\textwidth}
%     \centering
%     \includegraphics[width=.9\linewidth]{figs/temp/sw_speedup_4090.png}
%     \caption{Normalized kernel speedup on RTX 3060}
%     \label{fig:kernel_speedup_4090}
% \end{subfigure}



Fig.~\ref{fig:kernel_speedup} depicts the normalized speedup obtained on the backward pass alone. We observe a speedup of up to $5.7\times$ over baseline that uses butterfly reduction (\texttt{SW-B}). 
We observe a higher level of speedup on the RTX 4090, compared to RTX 3060. This is because the atomic bottleneck becomes more pronounced on the RTX 4090 when compared to the compute (containing 144 SMs and 176 ROP units, when compared to just 28 SMs and 48 ROPs in the 3060). 
We also observe that we achieve the highest level of speedup when the balancing threshold parameter is set to a parameter in-between the extremes. This shows that setting $0$ or $32$ as the balancing threshold leads to a bottleneck developed in sub-core or ROP units respectively.


\begin{figure}[!htb]
\begin{subfigure}{0.49\textwidth}
    \centering
    \includegraphics[width=.9\linewidth]{figs/temp/sw_speedup_4090.png}
    \caption{Normalized kernel speedup on RTX 3060}
    \label{fig:kernel_speedup_4090}
\end{subfigure}


\begin{subfigure}{0.49\textwidth}
    \centering
    \includegraphics[width=.9\linewidth]{figs/temp/sw_speedup_3060.png}
    \caption{Normalized kernel speedup on RTX 3060}
    \label{fig:kernel_speedup_3060}
\end{subfigure}

    \caption{Normalized kernel speedup on different models and workloads.}
    \label{fig:kernel_speedup}

\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/temp/w_wo_prim_SWS_speedup_4090.png}
    \caption{Normalized speedup with and without primitive index on 3DGS with RTX 4090.}
    \label{fig:wwo_prim_speedup}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/temp/w_wo_prim_SWS_einsn_4090.png}
    \caption{Normalized increase in total number of executed instructions with and without primitive index on 3DGS with RTX 4090.}
    \label{fig:wwo_prim_executed_instructions}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=.9\linewidth]{figs/temp/sw_real_speedup.png}
    \caption{Normalized end-to-end speedup on RTX 4090 and RTX 3060.}
    \label{fig:end_to_end_speedup}
\end{figure}



\subsection{SW bottleneck analysis}



\textbf{Stall count}
Fig.~\ref{fig:warp_stall_sw} shows the number of warp stalls per instruction on an RTX 4090 GPU. We observe that with \texttt{SW-B} stalls due to LSU contention are alleviated, and are fewer than $\%$  of the overall stalls.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=.9\linewidth]{figs/temp/perc_atom_stalls_sw.png}
%     \caption{Number of warp stalls per instruction (RTX 4090).}
%     \label{fig:warp_stall_sw}
% \end{figure}


\textbf{Instruction count vs atomic operations}
Fig.~\ref{fig:instruction_count} measures the number of atomic instructions issued vs instruction count normalized to the baseline. We observe that on increasing the balancing threshold parameter, the number of instructions to be executed by the sub-core increases, which contributes to the bottleneck compute bottleneck in the SM. The number of atomic operation requests decreases, alleviating the bottleneck caused due to atomic operation contention. 
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/temp/sw_balance_factor_4090_3DGS.png}
    \caption{Normalized speedup with varying balance factor $b$ on 3DGS with RTX 4090.}
    \label{fig:balance_factor_4090_3dgs}
\end{figure}


\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/temp/sw_balance_factor_4090_nvdiff.png}
    \caption{Normalized speedup with varying balance factor $b$ on \texttt{Nvdiffrec} with RTX 4090.}
    \label{fig:balance_factor_4090_nvdr}
\end{figure}
\textbf{Primitive reduction}
\label{sec:results_cccl}
In Fig.~\ref{fig:wwo_prim_speedup}, we depicts the speedup normalized over baseline on the backward pass for \texttt{SW-B} and \texttt{CCCL} respectively.
We observe a significant speedup (of up to 4X) on updating evaluating the reduction operation on all parameters in a loop. This is because updating each parameter with a separate reduction routine produces several instructions by the compiler. The number of instructions executed is depicted in Fig.~\ref{fig:wwo_prim_executed_instructions}. 
% We see that calling individual reduction function calls requires a significantly more instructions to be executed.


% \begin{figure}[!htb]
%     \centering
%     \begin{subfigure}{0.235\textwidth}
%     \includegraphics[width=\linewidth]{figs/temp/insn_red_3DGS_playroom_4090_SWS.png}
%     \caption{SW-S Playroom}

%         \end{subfigure}
%     \begin{subfigure}{0.235\textwidth}
%     \includegraphics[width=\linewidth]{figs/temp/insn_red_3DGS_playroom_4090_SWB.png}
%     \caption{SW-B Playroom}

%         \end{subfigure}

%     \centering
%     \begin{subfigure}{0.235\textwidth}
%     \includegraphics[width=\linewidth]{figs/temp/insn_red_3DGS_lego_4090_SWS.png}
%     \caption{SW-S Lego}

%         \end{subfigure}~
%     \begin{subfigure}{0.235\textwidth}
%     \includegraphics[width=\linewidth]{figs/temp/insn_red_3DGS_lego_4090_SWB.png}
%     \caption{SW-B  Lego}
%      \end{subfigure}    
   
%     \caption{Executed instruction count and number of atomic operations in relation to the balance factor on {3DGS} with RTX 4090.}
%     \label{fig:instruction_count}
% \end{figure}




\subsection{Speedup of \projname-HW}
Fig.~\ref{fig:hw_speedup_3dgs} and \ref{fig:hw_speedup_nvdiff} shows the speedup obtained with respect to baseline of \texttt{\projname-HW} on. We observe an average speedup of $5\times$ over baseline approach, and $\times$ \todo{adrian: enter exact values} over  \texttt{AB}.
% We see that \projname-HW performs better than the SW approach, as it eliminates the control flow overhead introduced by the programmer in the software approach, and does not require any additional hyperparameter tuning.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.7\linewidth]{figs/temp/hw_3dgs_playroom.png}
%     \caption{Normalized speedup on hardware simulator that emulates RTX 4090 and RTX 3060 on 3DGS Playroom with SM reduction and our SCAR-HW.}
%     \label{fig:hw_speedup_3dgs}
% \end{figure}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.7\linewidth]{figs/temp/hw_nvdiff_bob.png}
%     \caption{Normalized speedup on hardware on NVDiff Bob.}
%     \label{fig:hw_speedup_nvdiff}
% \end{figure}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.7\linewidth]{figs/temp/hw_nvdiff_lego.png}
%     \caption{Normalized speedup on hardware simulator that emulates RTX 4090 and RTX 3060 on NvDiff Lego.}
%     \label{fig:hw_speedup_nvdiff}
% \end{figure}

\subsection{Energy analysis}
\label{sec:energy_analysis}
Fig.~\ref{fig:energy_consumed}. We observe that \projname delivers on average $5.6\times$\todo{adrian: put the exact number} energy savings.
Fig.~\ref{fig:interconnect_traffic} shows the interconnect traffic change in using \projname-HW in various workload - dataset configurations measured on NVIDIA RTX 4090, in which we observe a reduction in the interconnect traffic. We observe that
\projname requires fewer memory I/O requires (atomic requests) to be issued from the via queue to the memory sub-partition. As each memory issue through the interconnect requires consumes a significant amount energy (compared to the computation, which is equivalent in our case), \projname-HW saves energy significantly in this regard.
 % The corresponding overall energy consumed is visualized in 

% \begin{figure}[!htb]
% \begin{subfigure}{0.49\textwidth}
%     \centering
%     \includegraphics[width=.5\linewidth]{figs/temp/hw_power.png}
%     \caption{Normalized reduction in energy consumed by the backward pass.}
%     \label{fig:energy_consumed}
% \end{subfigure}

% \begin{subfigure}{0.49\textwidth}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/temp/sm_l2_traffic_red_4090.png}
%     \caption{Normalized reduction in total SM $\rightarrow$ L2 interconnect traffic in the backward kernels on RTX 4090.}
%     \label{fig:interconnect_traffic}
% \end{subfigure}

% \caption{Analysis of energy consumed}

% \end{figure}


==> text_srcs2/introduction.tex <==


Differentiable rendering leverages machine learning to solve some fundamental tasks in computer graphics, such as scene reconstruction~\citep{nerf, 3dgs} (deriving a representation of a 3D scene),
and inverse rendering~\cite{mitsuba, nvdiffrec} (estimating shape, texture, lighting, and material of a 3D object) from a set of rendered/captured reference images.
These problems are central to many important applications~\cite{tewari2020state}, such as photogrammetry, 3D modeling and scanning, 3D model creation tools, game engines, and AR/VR applications. 
With differentiable rendering, these tasks are formulated as a learning problem that can be solved using gradient descent-based optimization techniques. 

For example, 
% neural rendering is a popular and promising approach that capture real and photorealistic  
neural radiance field (NeRF)~\cite{nerf, instantngp, tancik2023nerfstudio, mipnerf360, zipnerf,tensorf, bakingnerf, nsvf, plenoctrees, dvgo, plenoxels}
is a popular and promising approach to synthesizing novel views of 3D scenes. NeRF represents a scene as a 3D volume field parameterized by neural networks/features. 
% Any 2D view of the scene can then be rendered using this representation. 
% These learnable parameters are trained to represent a scene using gradient descent by computing a loss function between a ground truth image and the image generated by rendering the current model. 
These neural parameters are trained with gradient-based optimization to minimize the difference between ground truth images and images differentiably rendered with NeRF. 
% A differentiable renderer is used to compute the loss gradients with respect to these scene parameters.  
Learning-based methods for these tasks have demonstrated significant success in achieving state-of-art quality in scene reconstruction, leading to huge interest in the computer graphics, vision, and robotics communities. This success has led to the development of several specialized frameworks and libraries for differentiable rendering~\cite{nvdiffrast, pytorch3d, mitsuba, drjit}, and recent work~\cite{slang, slangd} propose native support for differentiable rendering in GPUs as a first-class feature. Prior works~\cite{li2022rt, neurex, instant3disca, artist,  mubarik2023hardware} have also proposed accelerators for NeRF-based rendering and training. 

% 
Another line of work for differentiable rendering is to leverage the high-speed rasterization pipeline~\cite{opengl}. Rasterization requires the scene to be represented as a set of \emph{geometric primitives} (i.e. meshes, triangles, points) in 3D space which can then be rendered as 2D images with very high speeds. %This set of geometric primitives can make use of the high-speed rasterization pipeline~\cite{opengl} in GPUs to be efficiently rendered on screen. 
Differentiable rendering with rasterization involves learning these primitives using similar gradient descent-based training. This approach~\cite{pulsar, nvdiffrec, adop, 3dgs} has demonstrated state-of-art capability in producing high-quality scene reconstructions at high speeds and emerged as a fundamental representation of 3D visual data. 
%has emerged as very promising due to the high speed rendering and the ability to learn high quality representations of the scene. 
%has increasingly becoming a popular technique for learning-based tasks, after several recent works~\cite{pulsar, nvdiffrec, adop, 3dgs} on these aforementioned tasks.
% A widely-used scene representation method to encode visual information is to consider the scene as being composed of a large set of geometric \emph{primitives} in 3D space (i.e. triangles, points, voxels). Each primitive is associated with color information. 
%%%%%%%%%%%%%%%%% RF: may need one sentence to connect
% This raster-based differentiable rendering method is efficient as these primitives can be rendered on screen using a high-speed rasterization pipeline~\cite{opengl}. 
% Several recent works~\cite{pulsar, nvdiffrec, adop, 3dgs, 4dgs, dynamic3dgs} incorporate differentiable raster-based renderer in learning each primitives' parameters (position, color, etc.) on these aforementioned tasks.  
Among these methods, a recent transformative work, 3D Gaussian Splatting (3DGS)~\cite{3dgs} has spurred significant interest in both industry and academia~\cite{3dgs_avatar, dynamic3dgs, deform3dgs, 3dgsdreamer, 3dgs_flexiblerendering, 4dgs, gaussianrep_survey}.
%in the computer graphics community. 
3DGS represents the scene geometry with 3D Gaussians as its primitives % (that are associated with learnable parameters) %, and associates each Gaussian with a view dependent color.
and uses an efficient tile-based rasterizer~\cite{adop, pulsar} with alpha-blending to render images from 3D Gaussians.  
% The sheer level of success of this method led to its adoption in Unreal Engine~\cite{unreal}.
%Owing to the speed and quality advantages inherent in these methods, differentiable rendering using raster-based pipelines has established itself as a promising approach for the future.

% To investigate the existing limitation of raster-based differentiable rendering methods and advance towards faster differentiable rendering, we performed comprehensive profiling on several important differentiable rendering workloads using state-of-the-art raster-based methods. 
While rendering scene representations with learnable parameters can be done at high speeds using the raster-based rendering pipeline, \emph{training} these models to learn scenes is still much slower compared to forward rendering.
% or x times slower compared to forward rendering.
% \emph{training} these models to learn scenes is still a slow process requiring a several hours for each scene on a powerful GPU. 
In this work, we perform a detailed performance analysis of differentiable rendering applications. This computation involves a forward pass (rendering an image), loss computation, and gradient computation (computing gradients with respect to trainable scene parameters) and applying gradient updates to these learned parameters.
We find that the gradient computation step of the backward pass is a significant bottleneck. For example, in \texttt{3DGS} workloads (see~\cref{sec:methodology} for details), we find that the gradient computation kernel takes up on average 30.07\% (up to 65.8\%) of the overall training time on the NVIDIA RTX 4090 GPU (\cref{sec:motivation_backward_runtime}).

% Hence, in this work, we focus on these raster-based differentiable rendering implementations for GPUs, which constitute a family of widely methods for 3D scene reconstruction and inverse rendering tasks.
Our analysis shows that this bottleneck is primarily caused by a large number of atomic operations that accumulate gradients for the trained parameters. During the gradient computation, each thread is associated with one pixel. It computes and accumulates the parameter gradients for all primitives the pixel is associated with. %As different pixels can be influenced by the same primitive, the gradient update for each primitive parameter are performed with atomic operations to avoid racing conditions across the threads. 
These gradient updates must be done using atomic operations since multiple threads may update the same parameters.
This leads to a massive number of atomic operations being launched by each thread.
%, since each pixel is influenced by a set of primitives with trainable parameters. 
These atomic operations cause significant contention at the atomic units at the L2 memory subpartitions (ROP units), leading to long stalls at the GPU streaming multiprocessors (SMs) (~\cref{sec:motivation_shaderbwdimpl}).

% Hence, each pixel is associated with a large number of primitives, and each primitive has many parameters.

Our \textbf{goal} in this work is to accelerate raster-based differentiable rendering applications by accelerating atomic operations that constitute a significant bottleneck during the gradient computation. 
% One possible approach to alleviate the bottleneck due to atomic reduction operations is to offload some of the the atomic reduction computation locally to the SM. 
% This is possible to do when several threads executing within the SM atomically update a same addresses. 
From our analysis of atomic operations in gradient computation, we make two observations: \textbf{(1) Locality in intra-warp atomic updates:} Threads \emph{within a warp} typically update the same parameters and thus the \emph{same memory location}. For example, on the \texttt{3D-PR} workload (see~\cref{sec:methodology} for details on workload-dataset configurations), we find that over 99\% of warps have all its threads update the same memory location  (\cref{sec:motivation_observations}).   
%This leads to a large number of threads within a warp to add gradient updates to the same set of memory addresses via atomic requests. 
\textbf{(2) Only a subset of threads in a warp perform atomic updates:} There is significant variation in the number of threads within each warp that make gradient updates at any time (~\cref{sec:motivation_observations}) as some threads are made inactive due to failing condition checks in the code (i.e., control divergence). The number of threads making atomic requests determines the atomic request traffic generated by the warp and varies across warps.
%This means that different warps contribute a different level of atomic request traffic in the instruction queue.

%We leverage Observation 1 to reduce the traffic of atomic requests by aggregating atomic add operations to a common address at the sub-core level first, and issue a single atomic add request on the result of this summation. This will completely clear up traffic of atomic requests on the memory instruction queue and would lead to underutilization of atomic computation units (ROP units) at the memory subpartitions. 
%To improve the utilization of the ROP units, we schedule a fraction of warps to do reduction computation in the ROP units. Which warps' computation gets scheduled to the ROP units is determined by the amount of atomic request traffic the warp contributes to. 
%Based on observation 2, different warps contribute a different amount of atomic request traffic to the instruction queue. We dynamically identify warps with low contribution and schedule their atomic requests directly to the ROP, skipping the sub-core level reduction.

% Bottlenecks caused due to high atomic request traffic is common in remote memory operation (RMO) architectures (like GPUs)~\cite{fermiarch, rmo, t3ermo}. General approaches that focus on atomics processing in GPUs architectures alleviate this memory traffic using general approaches either propose novel cache coherence protocols GPU~\cite{gpucachecoherence, atomiccoherence, acceleratingatomics}, or change the memory consistency model~\cite{}. For works in which threads executing in the SM update the same parameter (as is the case in raster-based differentiable rendering - from observation \textbf{(1)}) In works that using the bottleneck caused due to atomic memory traffic~\cite{bssync, lab, massiveatomics, acceleratingatomics} fall into two categories:  to alleviate bottlenecks  

Prior approaches~\cite{lab, phi, hlrc} that address bottlenecks due to atomic requests in GPUs, buffer and aggregate atomic updates in the L1 cache to reduce traffic in the interconnect and L2 atomic units (ROP units). 
%These buffered atomic updates are aggregated and written back to L1/shared memory itself and are only \emph{evicted} (make a global atomic update) when the buffer exceeds capacity.
While these approaches can effectively alleviate overheads from atomic operations for a wide range of applications, they do not leverage the intra-warp locality in atomic updates seen in differentiable rendering. The sheer number of atomic requests generated also overwhelm the load-store units before the atomics can be aggregated, making this approach less effective for differentiable rendering workloads (see ~\cref{sec:results_hw_performance} and~\cref{sec:related_work}). 

%However, we find that the bottleneck in raster-based differentiable rendering workload results from the rapid rate at which atomic requests are issued by each sub-core of the SM, causing contention at the SM's load store unit (LSU, which handles memory instructions to/from the SM) itself. Prior works do not alleviate the bottleneck due to slow atomic processing and memory operations at the L1/shared memory level in these applications. 

In this work, we introduce \projname (\underline{S}ub-\underline{C}ore and \underline{A}tomic-Unit collaborative \underline{R}eduction), a primitive that accelerates atomic
updates in applications that (1) generate significantly large amounts of
atomic requests and (2) typically have
most threads within an warp performing atomic updates to
the same memory locations. 
%

\projname is based on two key ideas: \textbf{(1)} We leverage intra-warp locality in atomic updates (Observation 1) to perform \emph{warp-level reduction} at the core itself using registers. This significantly reduces the number of atomic operations that need to be sent to the L2 atomic units to update global memory. \textbf{(2)} We dynamically distribute the atomic computation between the cores and L2 atomic units to enable high throughput atomic updates by leveraging all atomic units. Leveraging Observation 2, warps that only a generate a few atomic updates are handled at the L2 atomic units. Warps where most/all threads generate atomic updates are first reduced at the SM using the proposed warp-level reduction.
Implementing \projname requires addressing important design challenges (described in~\cref{sec:design_challenges}). We propose two implementations of \projname: 

\textbf{\projname-SW}. This software-only approach leverages existing warp-level  primitives (such as \texttt{\_\_shfl\_sync}) to implement warp-level reduction at each SM sub-core. All atomic updates to any memory location involving more than a predefined number of threads in a warp is performed at the SM, and the rest is performed at the ROP units. This predefined number is a tunable hyperparameter (the \textit{balancing threshold}).
%, to perform opportunistic sub-core level atomic reduction. It dynamically detects the number of threads in a warp that actively participates in an atomic operation with common addresses. It performs warp-level aggregation when this number is larger than the balancing threshold. We implemented \projname-SW with existing warp-level programming primitives (such as\emph{\_\_shfl\_sync}) to enable atomic reduction at sub-core level, even when only a subset of warp threads actively participate in the reduction.
% However, this approach requires hyperparameter tuning and a significant programming effort in implementing this solution. Additionally, the additional code introduced to do reduction at the sub-core level introduces additional control flow and compute latency overhead which could slow down the application.  

\textbf{\projname-HW}. %The additional code introduced to do reduction at the sub-core level introduces additional control flow and compute latency overhead which could slow down the application in software implementation. 
We propose a low-overhead hardware module in the GPU SMs to perform warp-level reduction using registers and leveraging the address coalescing unit. To distribute atomic computation between the SM and ROP units, we simply dynamically schedule based on their utilization. 
\projname-HW is exposed to the programmer using a new instruction. Compared to \projname-SW, this approach is more efficient as there are no overheads from additional instructions, redundant computation, and control flow, and it requires less programmer intervention (Sec.~\ref{sec:approach_hwdesign}). 
%hat adaptively selects either the sub-core or ROP units for reduction based on resource availability. 
%We modify the sub-core's instruction pipeline to process atomic reduction operations. As part of \projname's design, we introduce a new, low-overhead execution unit at each sub-core. This module contains an FP unit to perform the reduction and sends the result to the LSU instruction queue. \projname-HW's sub-core logic packs common atomic requests across different threads in a warp together into a single transaction. On issuing this transaction, \projname checks whether the LSU instruction queue is busy to issue requests to. If busy, \projname schedules the transaction to the reduction module to do the reduction.

We evaluate \projname across recent widely used differentiable rendering applications (3D Gaussian Splatting~\cite{3dgs}, NVDiffRec~\cite{nvdiffrec}, Pulsar~\cite{pulsar, pytorch3d}). With \projname-SW, we demonstrate a speedup of $2.60\times$ on average (up to $5.70\times$) for gradient computation and an average speedup of $\times$ (up to $2.4\times$) on the overall application on a real NVIDIA RTX 4090 GPU. With \projname-HW, we demonstrate an average speedup of $2.02\times$, and up to $4.69\times$ for gradient computation using a GPU simulator~\cite{gpgpusim}. Our contributions are summarized as follows: 
\begin{itemize}
\item This is the first work to perform a performance characterization of an important emerging workload, rasterization-based differential rendering for 3D visual data, and identify atomic updates as a key bottleneck.
\item We introduce \projname, a novel primitive to accelerate atomic processing in GPUs for applications that produce large amounts of atomic requests and with intra-warp locality in atomic updates. %We design and demonstrate the effectiveness of \projname on raster-based differentiable rendering applications to efficiently perform atomic reduction computation.
\item We propose two implementations: \projname-SW, a SW-only implementation, and \projname-HW, a low-overhead hardware implementation. We will open-source \projname-SW, which can be directly used to obtain significant speedups raster-based differentiable rendering workloads.
\item We evaluate \projname on popular differentiable rendering applications on both real hardware and using simulators and demonstrate significant speedups.
\end{itemize}
%We will provide an open-source, software implementation of \projname to readily accelerate raster-based differentiable rendering.








==> text_srcs_old/0_approach.tex <==
    
\todo{goal; accelerate inv. rend by accelerating - }
Our \textbf{goal} in this work is to accelerate raster-based differentiable rendering applications by accelerating the processing of atomic reduction operations which constitute a significant bottleneck in these applications. 
To this end, we introduce (i) \projname-SW approach, and \projname-HW |todo{a primitive that enables fast atomic operation reduction when 
 (1) ..... (2) ...... . In this work, we present SW and HW implementation of this primitive..} architecture design that selectively performs atomic operation reduction at the sub-core level to eliminate the atomic update bottleneck. \projname appropriately schedules reduction at the sub-core level as well as at the ROPs 
% send to ROP is not reduction? more like atomic passthrough
, based on the contention of resources at each unit.
% level atomic aggregation scene-parameter gradient computation in raster-based inverse rendering applications that have several threads computing the gradient of parameterized geometric primitives constituting the scene. These gradient components are then summed up (reduced) with atomic operations to produce the final gradient. 

% ADR edit: leverage the fact that several threads within a warp compute the gradient components of the same primitive to perform opportunistic aggregation and reduce the total number of atomic requests sent by each sub-core
The key idea of \projname is to (i) \todo{do } , to express the total gradient update computation to be done in-part by each warp, and a part at the memory partition units,\todo{long complex sentence} and (ii) minimize the time required to update several gradient parameters of the same primitive. 




%this sounds the same as point i?
A key challenge in distributing the computation across the SM core and the memory partition is managing the contention of compute resources at the L2 partition and the SM core. For instance, performing the entire reduction operation on a particular parameter in the SM core leads to a compute bottleneck on the FP units, leaving the ROP units at the L2 partition (where atomic operations are processed) idle, and vice versa.
To address this, we first outline our SW approach that computes a part of the reduction operation within the SM, and a part at the L2 unit. We describe how we can control the "amount" of reduction summation computation that is to be done at the SM vs the interconnect using a tunable hyperparameter.
We can then tune this hyperparameter to reduce the amount of idle time of the L2 ROP units and the FP units at the core.
% This parameter controls the ratio between warps that send atomics directly to L2 and warps that perform reduction.
\todo{maybe we mention interleaving?}

This approach, however, requires a significant engineering effort by the programmer and careful tuning in distributing this reduction computation. It also incurs additional overhead in performing branching instructions, leading to a slowdown \todo{diminished speedup}. To address this, we introduce \projname, a hardware mechanism that (i) adaptively tunes and manages the reduction  computation done at the L2 ROPs\todo{L2 ROP handle single atomic reqs} and the SM core (ii) requires no change in interface to the programmer (iii) eliminates the need for control flow instructions and redundant computation inevitable in SW, making it more power efficient\todo{making it faster?}. 

A high-level view of \projname is shown in Fig.~\ref{fig:distribution_reduction_high_level}. The reduction computation is completely performed in the SM core. The amount of reduction computation is adaptively controlled so that each resource is not kept idle.
% I think we should describe it as adaptively perform reduction when L2 ROP is occupied

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{figs/figure12.pdf}
    \caption{High-level overview of \projname}
    \label{fig:distribution_reduction_high_level}
\end{figure}


\subsection{Reduction Computation in the SM core}
% \begin{itemize}
%     \item Describe how reduction computation can be distributed
%     \item Provide mathematical equation for the reduction computation split
%     \item Describe what determines how much bottleneck is developed at each componetn - number of active threads doing the atomics overall - 
%     \item Mention that this depends on device, on application and dynamic parameters 
%     \item Describe our application profile.
% \end{itemize}
As described in Section~\ref{sec:key_observations}, each thread in the backward pass of the shader kernel computes a \todo{set of components?} component of the gradient of a parameter $x_i$ corresponding to a primitive $p$ , which we denote as $grad_t\_x_i$. The gradient of a parameter $x_i$ (denoted as $grad\_x_i$ ) of primitive $p$ is computed as a reduction (summation) of the gradient components computed by each thread as follows:
\begin{equation}
    p.grad\_xi = \sum_{t\in \mathcal{P}} p.grad_t\_xi
\end{equation}
Where $\mathcal{P}$ is the set of threads updating the gradient of parameters of the primitive $p$.
Each thread computes one term of this summation, and these terms are summed up to produce the total gradient with an atomic add operation. 
However, this results in a significant amount of time spent in evaluating atomic operations  
% is this just atomic bottleneck?
(Section~\ref{sec:key_observations}).

As several threads of each warp (which correspond to close by pixels) compute the gradient of parameters of the same primitive, we can alleviate the bottleneck by summing up the gradient of common parameters at SM\todo{Sub-Core?} level first, and then use a single atomic add operation on the result of the summation.
Within each warp, the threads summing to the same parameter can first be summed up at warp level as expressed below below:
\begin{equation}
    \label{eq:warpred}
    p.grad\_xi = \sum_{w\in \mathcal{W}} \sum_{t\in w(\mathcal{P})} p.grad_t\_xi
\end{equation}
where $\mathcal{W}$ is the set of all warps, and $w(\mathcal{P})$ is the set of threads in the warp updating the parameter $p$. The inner summation in Eq.~\ref{eq:warpred} can be computed within a single SM, using warp level primitives.

However, doing the reduction computation in the SM incurs an additional cost in control flow in finding the set of threads that update the same parameter before summing them. This adds a significant latency in evaluation of the atomic operation. We find that the cost of doing this might become significant bottleneck, and we show that it will ultimately slow up the application (Section~\ref{sec:results}).
% or maybe doing reduction trivially will slowdown the application

\subsection{SW approach}
\label{sec:approach_sw}
\todo{Would it be a better flow if we introduce SW-S first, then we identify the reasons for diminished speedup, }
\subsubsection{Controlling the Amount of Reduction Computation in SM vs L2 ROP units}

We need to ensure that the number of cycles spent in performing the reduction operation is the least it can be, before it becomes the main bottleneck. A reasonable method to modelling the latency required to the reduction at the SM-level is to count the number of floating point numbers that are required be summed up. We call this count, the "active count". 
This count is used to approximately model the latency of the reduction operation, as the active count parameter is monotonically related to the latency to compute the summation in the sub-core. Based on this "active count", we determine the appropriate location to do the warp level computation (the inner computation). Fig~\ref{fig:balance_threshold} demonstrates how the number of active threads leads to different latencies in doing reduction in each thread <todo>.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.5\linewidth]{example-image}
%     \caption{Microbenchmark of SM reduction latency with different active counts, vs ROP reduction latencies \todo{we're planning to remove this}}
%     \label{fig:balance_threshold}
% \end{figure}

We apply a threshold on this parameter to determine the appropriate location for doing the reduction.
We call this parameter the "balancing threshold", as it control the decision to doing reduction computation either in the SM core or the atomic units at the L2. Increasing the balancing threshold would lead to the longer latency reduction computation to be performed in the SM core while simultaneously freeing the bottleneck in the ROP units, and vice-versa. \todo{this is not true. Increasing balance threshold decreases overall number of reductions performed and increases total number of atomics sent to L2.}

\subsubsection{Factors influencing bottleneck in reduction computation}
The appropriate balancing threshold parameter depends on the level of contention of the L2 ROP units, as well as latency in doing reduction at the SM core. This is influenced by the amount of reduction operations to be performed, which in-turn depends on several factors, outlined below: 
\begin{itemize}
    \item \textbf{Dataset and workload type:} The amount of reduction computation to be done depends on the workload (scene representation primitives, camera resolution, etc.) and the scene data it's learning (detailed, large scale scenes with several primitives are slower to learn).
    % Different characteristics


% \begin{table}[!htb]
%     \centering
%     \begin{tabular}{c|c|c|c}
%         \textbf{Workload}     & \textbf{Atomic} & \textbf{Arithmetic} & \textbf{Best} \\
%         \textbf{}     & \textbf{Intensity} & \textbf{Intensity} & \textbf{Method} \\
% \hline
%         \texttt{gsplat}     & med  &  &  balanced   \\
%         \texttt{nvdiffrec}  & low  &  &  SM-reduce   \\ 
%         \texttt{pulsar}     & high &  &  serial-SM-reduce   \\

% \end{tabular}
%     \caption{Characterization of atomic intensity and arithmetic intensity of the workloads base don profile}
%     \label{tab:characterization_of_workload_and_method}
% \end{table}

    
    \item \textbf{GPU device architecture:} The different compute throughput of the GPU's SM cores vs the L2 ROP units influences the speed with which reduction computation that can performed. We test our approach on two different configurations: one with an RTX 3060 GPU configuration (low SM count compared to ROP units) and an NVIDIA RTX 4090 GPU (high SM count comprated to ROP units).
    
    \item \textbf{Reduction method used:}  Different methods of parallelizing the SM level reduction leads to different speedups, with a different set of trade-offs. In this work, we present two methods to do reduction in software, described below. 
\end{itemize}

% \subsubsection{\projname in Software}

% \begin{itemize}
%     \item Computation required to do reduction computation - mention what it depends on : check for common address for several atomic parameters
%     \item describe how this check can be done <once> - leading to speedup
%     \item Reduction can be performed in two ways - butterfly reduction and serialized reduciton, each with it's own tradeoffs and core contention profile.
% \end{itemize}


\subsubsection{\projname Serialized Execution}
% we hsould mention that this is a more general solution that do not require full convergence? Maybe we talk about butterfly first?
This approach requires looping through the computation of each operation.
The latency to do summation in this manner is proportional to the number of gradient parameters to be added. This approach however, is inefficient as a number of the summations can be parallelized. This incurs significant reduction in atomic latency as ...
A schematic of our software approach is shown in Fig.~\ref{fig:serialized_overview}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=.76\linewidth]{figs/figure14.pdf}
    \caption{Serialized reduction implementation overview}
    \label{fig:serialized_overview}
\end{figure}

\subsubsection{\projname butterfly reduction}
Fig.~\ref{fig:bfly_overview} shows an overview of the schematic used in the butterfly reduction. In this approach, we first check whether all the threads of the warp update the same primitive. If so, we use a reduction tree to compute the summation of each parameter.
This approach, however, requires all threads to be kept active. This means that the threads were originally inactive are required to sum an additional 0 value for the implementation.   
% This implies the programmer has to enforce convergence by keeping all threads alive and assigning 0-value gradients to threads that do not participate in the gradient update.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=.75\linewidth]{figs/figure15.pdf}
    \caption{Reduction-tree / butterfly reduction implementation overview}
    \label{fig:bfly_overview}
\end{figure}


\subsection{\projname - Hardware Design}
\label{sec:approach_hwdesign}

Our software approach has several limitations in executing a warp level primitive operations outlined as follows: 
% i is only true for SW-B. maybe we should talk about ii iii and iv as i ii iii and then mention i as an additional overhead for SW-Bs
(i) Incurs additional overhead in performing redundant computations in doing the reduction operation at the warp level, as only a fraction of all threads are producing actual updates every iteration. (ii) Introduces overhead with control flow instructions per thread in trying to do warp-level reduction (iii) Requires significant programmer and engineering effort in using warp level primitive instruction (iv) Requires careful tuning of workload and device-dependent hyperparameter to get the best-case speedup.

In order to address these issues, we introduce \projname, a sub-core level microarchitecture design to efficiently process the reduction summation operations for GPUs. \projname first finds groups of atomic instructions that update the same memory location by active threads in the warp. It then adaptively selects the appropriate hardware target (SM subcore or L2 ROP units) where summing-up operations are to be executed based on the level of contention, and schedules the reduction computation appropriately. If the L2 ROP units are selected, the reduce operations are directly scheduled in the same manner as atomic operations. If the SM subcore is selected, the gradient components from different threads re summed-up and the resulting sum is issued to L2 ROP units.
This ensures that the L2 ROP units are always kept busy during execution, while ensuring that it doesn't develop into contention.
% and lead to long stalls
Finally, in order to expose this functionality to the programmer, we encapsulate our sub-core reduction mechanism with a new warp-level instruction which we call "\atomred{}" instruction. Our modified GPU architecture schedules and decodes these \atomred instructions into one of the sub-cores.    
We implement our design by introducing three HW modules to the GPU sub-core microarchitecure to process these \atomred instructions: the \redcoalesce module, the contention determination module , and the \reduce module which picks up issued reduction operation. A high level overview of the design is shown in Fig.~\ref{fig:scar_high_level}.
% atomred is a seemingless swap from normal atomics
\begin{figure}[!htb]
    \centering
    \includegraphics[width=.75\linewidth]{figs/figure16.pdf}
    \caption{HW walkthrough of \projname \todo{this picture needs to change}}
    \label{fig:scar_high_level}
\end{figure}

\subsubsection{Atomic address coalescing}

The address coalescing module finds groups of active threads that point to the same memory address and coalesces them together to produce groups of \atomred request. This identification of common addresses is implemented using the same logic that is used to coalesce common memory addresses of all threads performing a load operation.

\subsubsection{Contention determination module (CD)}
The contention determination module receives reduction computation from the dispatch port (of each sub-core) of the load-store unit and checks whether. Is first checks whether the L2 interconnect queue is free to issue instructions into memory partition's ROP unit. If this queue is full, it  schedules the reduction operation to be processed by the reduction computation unit described below. 

\subsubsection{Reduction computation module}
The reduction computation unit contains a single floating point unit, which processes the summation computation of each group (coalesced unit) scheduled sum in a serial manner. 







==> text_srcs_old/0_detailed_design.tex <==
\label{sec:design_main}

In this section, we describe the specifics of the SW algorithm that explicitly expresses the reduction computation within the warp + atomic operations. We then outline the several limitations that this approach has, and we address them with our proposed \projname-HW design. We then describe each constituent component of a HW component, and their corresponding operations.

\subsection{Sub-core/ROP Level Collaborative Reduction in Software}
In order to implement our collaborative reduction approach in software, we need to design two main components: (1) type of reduction routine used that reduces at the warp level, and (2) criterion that determines whether the corresponding reduction is efficient to do at the warp-level or using atomic operations.
%normal atomic operations
Once these factors are determined, the overall process involves 3 steps: (i) Grouping the threads within the warp sharing a common parameter (ii) Determining whether the summation to a parameter in the warp and then sending out one atomic add operation is going to be efficient, or instead issuing several individual atomic add requests.
% If not, issue individual atomic add requests instead.
(iii) Performing the appropriate reduction computation based on the chosen approach. If the reduction on a parameter is performed at warp level, the resulting sum is then sent out with an atomic global update instruction. 

We present two methods to perform the sub-core level reductions, which differ in the method of warp level reduction operation used, and in requiring a different level of programmer effort: (1) where warp-reduction is performed in a serial manner (Section~\ref{sec:dd_serialized}), and (2) that does a parallelized summation of the reduction (described in~\ref{sec:dd_butterfly}). We describe the performance and programmer effort tradeoffs in the descriptions of these methods.

\subsubsection{Serialized Reduction}
\label{sec:dd_serialized}

Our SW approach is encapsulated using a device function that is called in place of the set of atomicAdd instruction in Algorithm~\ref{fig:atomicimplementation}. At each thread, the function receives a primitive index to be updated, the array of pointers to the primitive's parameters and the array of floating point values to reduce (see function prototype in Algorithm~\ref{alg:redserial}).

This reduction method perform warp-level reduction over a set of parameters corresponding to the same primitive explicitly, in a sequential manner. The REDserial algorithm is outlined in Algorithm~\ref{alg:redserial}. Groups of threads within a warp that update the same primitive's parameters are first noted using the "match\_any" warp instruction. Then, we determine a proxy for the latency in performing the reduction at the warp level. As mentioned in Section~\ref{sec:}, the decision is made by comparing a set threshold (called balancing-threshold) with the number of threads that are actively participating the current summation (this count is determined by the "popc" (population count) instruction). If the count is smaller than the balancing-threshold, the subcore's execution latency would then be considered to be higher than simply using atomic operations. In this scenario, the algorithm falls back to issuing native atomic instructions.
Otherwise, the reduction is performed by serially fetching and summing up each primitive parameter on each participating thread.
An advantage of this approach is that it is a drop in replacement of the atomic adds in  Algorithm~\ref{fig:atomicimplementation}, requiring no further code changes.

\textbf{Limitations:} The primary limitation of this approach is that the summation performed on to update common parameters is done sequentially, which adds to the latency of the reduction operation performed. Secondly, the list of parameters to iterate through for each unique parameter update iterating through the list of threads performing \emph{effectual} gradient updates adds to a list of. In addition, this approach introduces additional branching and control flow instructions adding to the overhead. 



% \begin{figure}[!htb]

% \colorbox[RGB]{239,240,241}{

% \begin{minipage}{.9\linewidth}
% \begin{algorithmic}

% \Function{BwdShaderSERIAL}{prims\_per\_thread}

% \State $tid \gets thread\_idx$
% \State $prims\_per\_thread \gets primitives[tid]$

% \For{ $p : prims\_per\_thread$}

% \If{ \Call{cond1}{} }
%     \State \textbf{continue;}
% \EndIf

%     \State ...    
% \If{ \Call{cond2}{} }
%     \State \textbf{continue;}
% \EndIf
%     \State ...    
%     \State \Call{red\_serial}{$p.grad\_{x1, x2,...xN}$,  $grad_{x1, x2,...xN}$}
%     \State ...    

% \EndFor

% \EndFunction
% \end{algorithmic}
% \end{minipage}

% }

% \caption{Outline of the shader's backward pass with RedSerial Implementation} 
% \label{fig:serialimplementation}

% \end{figure}



\begin{figure}[!htb]

\begin{lstlisting}
// 
template<typename ATOM_T>
void reduce_serial(int idx, ATOM_T** ptr, 
  ATOM_T *val, int num_params, int balance_thr) 
{
  int same_mask = "match_any"(idx);
  int same_ct = "popc"(same_mask); 
  if (same_ct >= balance_thrsh) {
    int leader = "ffs"(same_mask) - 1;
    same_mask &= ~(1 << leader);
    while (same_mask) {
      int src_lane = __ffs(same_mask) - 1;
      if (laneId==leader || laneId==src_lane) {
        for (int i = 0; i < len; ++i) 
          val[i] += __shfl(val[i], src_lane);
      }
      same_mask &= ~(1 << src_lane);
    }
    if (laneId == leader) {
      for (int i = 0; i < num_params; ++i)
        atomicAdd(ptr[i], val[i]);
    }
  } else {
    for (int i = 0; i < num_params; ++i) 
      atomicAdd(ptr[i], val[i]);
  }
}
\end{lstlisting}

\caption{Serialized SM-level atomic reduction \todo{RF: maybe we can add some vertical lines? since a lot nested if/loops}}
\label{alg:redserial}

\end{figure}


\subsubsection{Butterfly reduction}
\label{sec:dd_butterfly}
Motivated by the fact that a substantial percentage of warps have all their threads update the same primitive, and that the latency of reduction summation can be mitigated with a parallelized reduction tree, we propose a new approach that butterfly reduction, which we outline below. \todo{long sentence?}
Algorithm~\ref{alg:butterfly} presents the reduction algorithm that uses a reduction tree on all threads. This function has the same prototype as serialized version, except for a single exception - it receives a skip variable that indicates whether the current thread is skipping the atomicAdd operation or not. We first perform a check whether all the threads update the same address, and the number of summations performed is below the threshold (balancing\_thresh). If it's above the balancing threshold, we perform the summation over parameters using reduction-tree at warp level. Otherwise we send out several atomic add instructions.

\begin{figure}[!htb]
\begin{lstlisting}
// Input - primitive index idx
// output - 
template<typename ATOM_T>
void reduce_bfly(int idx, ATOM_T** ptr,
  ATOM_T *val, int num_params, int balance_thr, 
  bool skip) 
{
  // number of threads making nonzero updates
  int active_ct = "ballot"(skip); 

  // ensure all threads update same primitive
  bool all_same = "match"(idx) == 0xffffffff;

  if (all_same && active_ct >= balance_thrsh) {

    // reduction tree
    for(int offs = 16; offs >= 1; offs /= 2)
        val[i] += "shfl_down"(val[i], offset);

    // send result of warp level sum
    if (laneId == 0) 
      atomicAdd(ptr[i], val[i]);

  } else if (!skip) {
    // usual method = 
    for (int i = 0; i < num_params; ++i)
      atomicAdd(ptr[i], val[i]);
  }
}
\end{lstlisting}

\caption{Using butterfly reduction to do warp level reduction \todo{comments!}}
\label{alg:butterfly}






\end{figure}





% \begin{algorithm2e}[1]
% \caption{Another algorithm with caption}\label{alg:three}
% \KwData{Write here the required data}
% \KwResult{Write here the expected result}

% \eIf{condition}{
% instructions1\;
% instructions2\;
% }{
% instructions3\;
% }

 
%  initialization\;
%  \While{While condition}{
%   instructions\;
%   \eIf{condition}{
%    instructions1\;
%    instructions2\;
%    }{
%    instructions3\;
%   }
%  }
% \end{algorithm2e}


\textbf{Limitations:} The main disadvantage of this approach is that all threads are required to be kept active, regardless of whether they participate in the gradient accumulation or not. It requires significant changes to the kernel code by the programmer and may introduce inefficiencies at other parts of the code. This is unavoidable as dynamic butterfly reduction in software would introduce dynamic loop instructions, which slows down the execution significantly. As in Alg~\ref{alg:redserial}, this approach introduces additional branching and control flow instructions adding to the overhead.\todo{weird last sentence}


\begin{figure}[!htb]

\colorbox[RGB]{239,240,241}{     
\begin{minipage}{.9\linewidth}

% \begin{figure}

\begin{algorithmic}[1]

\Function{BwdShaderBFLY}{prims\_per\_thread}

\State $tid \gets thread\_idx$
\State $prims\_per\_thread \gets primitives[tid]$

\For{ $p : prims\_per\_thread$ }


\State skip = false;
\If{ \Call{cond1}{} }
    \State \textbf{skip = true;}
\EndIf
    \State ...    
\If{ \Call{cond2}{} }
    \State \textbf{skip = true;}
\EndIf
    \State ...    
    \State \Call{red\_bfly}{$p.grad\_{x1, x2,...xN}$,  $grad_{x1, x2,...xN}$}
    \State ...    

\EndFor

\EndFunction


\end{algorithmic}

\end{minipage}
}

\caption{Modified shader's backward pass with butterfly reduction} 
\label{fig:bflyimplementation}

\end{figure}

% \end{figure}


% \subsection{Hyperparameter Tuning}
% In our SW approach, we introduce a balancing threshold hyperparameter that determines whether reduction using warp instructions or using global atomics. The appropriate value for this hyperparameter is dataset, workload and device dependent, as outlined in Section~\ref{sec:approachhyperparameter}.

% In order to find the appropriate value for this, we propose a simple, lightweight method to tune this hyperparameter online. 

% <>

\subsection{HW design}

We design \projname-HW as an efficient architecture to schedule reduction computation at the sub-core level. \projname-HW adaptively performs sub-core level atomic reduction when ROP units are fully occupied. \projname-HW does not require any parameter tuning. It also provides swap-in replacement for existing atomic operations and does not require any additional programmer effort in changing the kernel code. This approach eliminates all control flow overhead introduced in computing the overall number of warp level parameters in the SW approach.


We first enable the programmer to expose the global atomic type reduction computation as a new assembly level primitive instruction, which we describe in Section~\ref{sec:programmer_interface}. This new instruction takes in memory addresses (where the result of the reduction is written to) as operands. These addresses of the threads of the warp are coalesced together such that common address targets are grouped together into a single transacton. This transaction is issued from the dispatch port of the load-store unit into a determination module, that determines which  to produce atomic  in   


We introduce 3 primary changes to the baseline GPU architecture to enable efficient processing of \todo{fill this}. 
The exact operation chosen depends on the level of contention of HW computation (L2 ROP units vs FP units).


\subsection{Programmer interface}
\label{sec:programmer_interface}
To enable programmers to access \projname's efficient reduction functionality, we provide an interface to it as a new thread-level instruction in the GPU's machine code. We indicate this as the \atomred assembly instruction, which has prototype is as shown below:


\centerline{\atomred \texttt{[\%addr],  \%f}}


Here, \texttt{\%addr} is memory location where the parameter resides, to which floating point number \texttt{\%f} is to be added. This prototype is similar to the baseline atomic instruction, except that there is not return type to the instruction.

\subsection{\atomred Address Coalescing}
\label{sec:design_redcoalesce}

Each sub-core of modern GPU architectures coalesce all addresses accessed each thread of a warp belonging to a single line into a single memory transaction. For baseline atomic operations, warp threads that access addresses (i) either different cache lines, or (ii) same cache line but overlapping cache blocks (4 bytes of cache line), are created into different memory transactions.
To handle the \atomred instruction, we modify this baseline coalescing architecture for the atomic unit to produce a new kind of memory transaction - the \emph{reduce} transaction. This transaction goes to a new instruction queue that is local to the subcore before being forwarded to the LSU instruction queue. The transaction has information of the list of cache block that are accessed by the atomic add instruction, along with the list of floating point values to be coalesced. 
Note that this address coalescing mechanism is the same as done for the global load operation in aggregating the request, except we add additional data to this transaction packet - the set of floating point values of each threads, and a 4 byte "mask" - which threads are producing the atomic add request.


\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/coalesce.drawio.pdf}
    \caption{Each local queue forwards an atomic transaction request to the local reduction queue}
    \label{fig:memory_transaction}
\end{figure}

These \atomred memory transactions, along with the regular memory requests are created at each sub-core level and are communicated via instruction queues to the ICNT interface (also known as memory I/O module) which contains the LSU queue (see Figure~\ref{fig:memory_transaction}). These requests are then sent to the ROP units via interconnect.


\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/detailed_desing_hw.pdf}
    \caption{Each local queue forwards an atomic transaction request to the LSU instruction queue}
    \label{fig:memory_transaction}
\end{figure}


We make use of the hardware coalescing module to implement the overall number of 



\subsection{Contention Determination Module}
\label{sec:design_contention_determination}
After the list of reduction transactions have been produced, these transactions are issued and enqueued into a new pipe in the sub-core that we introduce into \projname's design, which we call the sub-core reduction pipe. From this queue, our hardware needs to decide whether the reduction of operands of this transaction are to be done in the sub-core level, or they should be processed at the ROP units. This determination is done by the contention determination logic, \todo{indicated with the "queue/redunit empty?"label}. This unit first checks whether the LSU instruction queue is free or not. If the queue is free, it issues the transaction the same way as an atomic request to the LSU. If the queue is full, it checks whether the local floating point unit that performs reduction operation is free. If it is free, it schedules the reduction operation to this HW unit. The actual hardware used to perform the reduction is outlined in Section~\ref{sec:design_reduce}.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/hw_subcore.drawio.pdf}
    \caption{Each local queue forwards an atomic transaction request to the LSU instruction queue}
    \label{fig:subcore}
\end{figure}



\subsection{Reduction module}
\label{sec:design_reduce}

If the LSU instruction queue has contention in processing atomic operations, the contention determination unit selects the reduction hardware unit to perform the summation of parameters (see Figure~\ref{fig;subcore}). We design the reduction unit as a hardware module that performs the summation of floating point parameters of different threads of a warp that point to the same address. Figure~\ref{fig:hw_reduction} shows our design. The unit receives the transaction information indicating teh mask of the threads of the warp whose corresponding parameter values are to be summed up, and the corresponding floating point operands as input. The module's control logic serially goes through the active parts to compute the result as shown. This result is then forwarded to the LSU instruction queue.

\textbf{Note:} Although it is possible to utilize the FP units of the sub-core itself to perform this summation operation, we found that using just a single additional floating point unit (which incurs low overhead) per sub-core would be able to reduce the atomic request contention significantly.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.6\linewidth]{figs/reduction.drawio.pdf}
    \caption{Reduction computation unit, which serially computes the reduction result from }
    \label{fig:hw_reduction}
\end{figure}





\subsection{Overheads Analysis}
\label{sec:overheads_analysis}

To estimate the area overheads of implementing the \projname's hardware improvements, an open source implementation of the floating point unit\cite{hardfloat} was used. The unit was synthesized using the yosys\cite{yosys} synthesis suite for a generic cmos technology to obtain the transistor count of approximately $60,000$. The proposed changes introduce one floating point unit per-shader subcore. Considering a modern GPU architecture like NVIDIA RTX 4090, which has 4 subcores per SM and 144 SMs and $17.8$ billion transistors, \projname introduces an area overhead of $0.2$\%.




% The \projname's hardware implementation introduces one floating point unit per-shader subcore. To estimate the overheads
% Considering a modern GPU architecture like NVIDIA RTX 4090, which has 4 subcores per SM, and 144 SMs, we estimate the overehad in introdu






==> text_srcs_old/0_introduction.tex <==

\begin{itemize}
    \item \textbf{Motivation and intro:} Graphics processing units (GPUs) trace their inception as an accelerator to render a 3D scene containing several objects in it into an image to be displayed on screen.
    \item An adjascent problem, known as "inverse rendering", involves deriving properties of the 3D environment (such as geometries of objects, color, material properties, etc.) from a set of images captured by a set of cameras overlooking the scene.
    \item This scene representations are used in several current and upcoming applications such as photogrammetry, 3D modelling and scanning, 3D model creation tools, game engine designs, AR/VR applications, etc. 
    \item Inverse rendering has gained particular attention in recent times, after recent work demonstrated success in applying gradient-based optimization techniques and accelerating the algorithms by leveraging general-purpose GPU computation for acceleration~\cite{3dgs, pulsar, nvdiffrec, dmtet, flexicubes, instantngp, dvgo, plenoxels, nerf, neus}.
    \item For example, a recent and notable work in doing state-of-the-art 3D scene reconstruction, which learns scene parameters insanely-fast is 3D gaussian Splatting~\cite{3dgs}. Recent methods have already been applied to Unreal Engine~\cite{unreal}, a mature tool used as a 3D modelling application and a game engine. 

    \item As a result of recent interest in inverse rendering techniques, there is a growing trend to incorporate support in GPUs as a first class feature, similar to rendering~\cite{slang}.  

    \item \textbf{Explain how inverse rendering is done:} Inverse rendering typically producing an image from a parameterized scene representation, and comparing this with a corresponding ground truth image taken for the scene. A loss function can be computed which measures the difference between the ground truth image and the rendered image.

    \item This loss function is minimized by backpropagating the loss derivative to obtain the derivative with respect to the scene parameters, and then applying gradient descent on these parameters.

    \item In order to do this, the renderer operations of differentiable renderer, in which each operation of the rendering algorithm is differentiable, and can be backpropagated.


    \item Traditional raster-based rendering pipelines consider the scene of being comprised of several fundamental physical objects, or "primitives", in 3D space (such as a mesh composed of triangles, point cloud, spheres, etc.), each one associated with a color map / texture. These primitives are rendered as seen by a camera on screen using the rendering pipeline, which consists of 2 main stages: 1) \textbf{rasterization}: to find the list of primitives that are going to affect each pixel of the rendered image, and 2) \textbf{fragment-shading} - to determine the color each pixel in the rendered image by blending the radiance component of each primitive.

    \item \emph{Differentiable} raster-based rendering pipeline adds two additional fundamental routines: 1) backward rasterization - which is functionally similar to rasterization, and 2) backward shading: which takes as input the derivative of a certain loss function with respect to each of the pixel's color channel and computes the gradient of the parameters defining each primitive's location, shape and texture with respect to a loss function.

    \item Out of these stages, a vast amount of work in computer graphics literature over the years focused on optimizating the rasterization stage SW~\cite{opengl, tiled_rasterization, zbuffering} and fragemnt shading stage~\cite{texturemem, }.

    \item \textbf{Explain how differentiable shading constitutes a bottleneck in several of these works:} 

    \item Backward-pass of shading routine, however, constitutes a significant bottleneck in the overall rendering pipeline.
    \item This routine takes up as much as 30-90\% of the overall time required to do inverse-rendering workloads. 
    \item Both the forward pass and backward pass of the shader routine, consist of embarassingly parallel routine that either (i) independently computes the color of each pixel in the forward pass, or (ii) computes the gradient contribution of each primitive affecting each pixel. 
    \item However, unlike the shader's forward pass which \emph{independently} computes the color of each pixel, the backward-pass of the shader routine requires of aggregating the contribution of the gradient to each primitive of each pixel's gradients update of scene parameters. This involves aggregating the gradient contribution of each pixel's loss computed by each thread. 
    
    \item This fundamentally requires communication across threads in updating the gradient parameter, requiring the need for synchronization routine between them. These gradient updates are independently updated using atomicAdd operations in the rendering routine for \emph{each} of these operations.

    \item Each thread in the backward pass makes several atomic requests. The number of atomic requests grows rapidly with image size (proportional to the number of pixels / quadratically with the resolution), and linearly with number of primitives contributing to the gradient of each gradient. This number can be as high as several 10s of millions of operations for a high resolution image. 
    \item Based on our profiling results, we observe that atomic operations constitute the primary bottleneck in the shader's backward pass.
    \item This bottleneck arises because of serialization of execution of atomic operations at the l2 level, at the rop units.

    \item \textbf{List the key observations: locality, skipping \emph{ineffective} updates in aggregation, unique index involved in atomic aggregation.}
    \item On analyzing the nature of the atomic operations launched by the shader's backward pass, we make the following key observations: \textbf{(1) Locality in updates of atomic operations:} A large number of threads of each warp do gradient updates to the same memory address via atomics. In fact, we find that the number of warps having all its threads updating the same addresses are up to 95\% in certain applications. This happens because the threads of a warp correspond to close-by pixels of the image, and the accumulate gradients of each primitive and each primitive influences affect a local set of pixels. \textbf{(2) Several atomic accesses can be indexed by the same identifier:} Each primitive is parameterized by several parameters. Updating each parameter requires a unique atomic request to be generated. Each of these atomic acquires a lock on memory locations corresponding to each of these parameters. However, all atomic gradient updates of parameters of a single primitive can instead be updated by acquiring a lock on a single index corresponding to the primitive being updated, \textbf{(3) Skipping of ineffective updates by several threads:} only a fraction of the threads send out atomic addition requests for gradient updates. We call these threads \emph{effectual} threads. The remaining fraction of threads either enter a branch of execution that thread avoid sending out atomic add requests, or atomically add a $0$ value to the gradient (\emph{ineffectual} threads). Whether a thread is going to send an atomic update or not is determined dynamically by the backward rendering algorithm.  

    \item \textbf{talk about SW approach prior works}
    To alleviate the atomic bottleneck, one possible approach to leverage the locality in atomic updates is to first reduce all atomic requests (updating the same address) within a warp / SM-level first, and then send out a single atomic request updating the result corresponding to each unique address. However, we observe that doing this in software will introduce a significant number of instructions and control flow, which can slow down execution. significantly. 
    \item \textbf{Talk about atomic fusion - hardware approach}
    Prior hardware approaches, such as atomic buffering (LAB~\cite{lab} and DAB~\cite{dab}), propose a technique to fuse atomic requests of each warp on atomics updating the same address dynamically by coalescing and computing the sum in each SM. However, doing complete reduction would lead to development of a new bottleneck from atomic requests at L2 to compute intensity in the core in doing reduction.   

    \item \textbf{Goal:}
    \item Our \textbf{goal} in this work is enable fast execution of the parameter gradient update step of the shader's backward pass routine, which is useful to speedup several inverse rendering applications. To this end, we introduce \projname, a mechanism that leverages the locality in the atomic updates produced by the threads of each warp to offload a portion of the computation to the  . The key idea of our approach is to and application shading  of atomic reduction operations in a distributed manner by between the SM cores and the memory controller collectively, such that are not kept starved from processing. We do this by (i) Aggregating common address within a warp per SM, and sending collectively (ii) Sending out atomic operations only when required.

    \item \textbf{Key Idea: <>}
    \item In this work, we introduce \projname, a mechanism to leverage locality of atomic updates to allow warp-level reduction to alleviate the bottleneck. The key idea of our work is to distribute the processing of atomic operations between the ROP units and the SM core.

    \item \textbf{Main Proposal:}
    \item We propose - 
    \item \textbf{(1)} 2 SW-approaches to distribute the computation of atomic reduction processing across the ROP units at L2 level and the floating point units of the SM core. These approaches do a warp-level reduction by using warp level primitives (such as\emph{\_\_shfl\_sync}) to access thread data from different warps and then aggregating them using FP unit (+ operation). As each thread has to update several parameter of the primitive, this requires a check across warps to find the common address for each parameter. To alleviate this checks in doing reduction, the single primitive index for aggregation. Several update parameters (that update several parameters of a single primitive can be done by using atomic ) 
    \textbf{(1)} Our first SW mechanism works well in scenarios with \emph{strong} locality, where all atomic update addresses of all threads are the same. This approach does a butterfly reduction of all atomic operations in a single warp on a fraction of the warps, and the remaining fraction send out atomic request in the regular manner.
    - Our second SW mechanism works well under \emph{weak} locality, where fraction of atomic update addresses of all threads. This approach is similar to the first one, with one critical difference: we aggregate the atomic update serially instead of doing a butterfly reduction.     
    \item \textbf{Limitations of SW approach:} 
    The software approach requires the programmer to specify parameters that distribute the computation across ,. Additionally, it is now the duty of the programmer  introduces control flow  
    \item \textbf{(2)} To solve this,  We then propose a HW approach the ...
    % \item The memory consistency semantics for atomicAdd primitive involves an acquire-release semantics which guarantees the 

    \item High cost of reduction. this shifts the bottleneck of execution towards the SM floating point execution.
    

    \item Our list of contributions can be summarized as follows: 

    \begin{itemize}
        \item We provide a detailed characterization of rasterization + shading based on a wide range of inverse rendering workloads
        \item We provide a detailed characterization of rasterization + shading based on a wide range of inverse rendering workloads
    \end{itemize}

\end{itemize}






==> text_srcs_old/0_motivation.tex <==
% \subsection{Inefficient Backward Pass}
% \todo{change title: look at other papers "ineff. bwd pass"} 
\label{sec:motivation_backward_runtime}
% As described in Section~\ref{sec:bckg_diffrendering}, the forward pass of the raster-based rendering pipeline involves first rendering an image from a parameterized scene representation. A loss is then computed as the difference between the rendered image and the ground truth. On backpropagating this loss, we can find the gradient of the loss with respect to the scene parameters, enabling us to perform gradient based optimization on these scene parameters.

In this section, we profile key raster-based differentiable rendering workloads and Fig.~\ref{fig:backward_runtime} depicts the breakdown of how much of the execution time is spent in different parts of the overall computation (see Section~\ref{sec:methodology}), including the forward pass, loss calculation and the backward pass.
We observe that up to \todo{} $60\%$  of the total runtime is spent on the backward pass, showing that the backward pass constitutes a significant bottleneck. 

% \todo{several small bars with lowest blue bar depicting bwd} 


\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/temp/perc_backward_kernel.png}
    \caption{Percentage of time spent on backward pass of the shader during training}
    \label{fig:backward_runtime}
\end{figure}



\subsection{Atomic Reduction Bottleneck in the Backward Pass}
\label{sec:motivation_shaderbwdimpl}
% \subsection{Implementation outline of the backward shader kernel}

% Here, we inspect the backward shader kernel in further detail. \todo{is this professional?}
The input to the backward pass is a set of per-pixel lists of primitives that influences the color of the corresponding pixel (discussed in Section~\ref{sec:bckg_diffrendering}). The backward pass iterates through this list of primitives to compute the gradients of each primitive for each pixel. This is an embarrassingly parallel computation that is trivially parallelized across pixels, with each thread performing the computation for one pixel. The gradient computation in the backward pass of differentiable rendering workloads is depicted in Alg.~\ref{fig:atomicimplementation}. 
% the gradient of a loss function with respect to parameters of scene primitives, from the gradient loss with respect to the pixel color channels.
% Each thread receives a list of primitives as input and computes the gradients of the parameters of each primitive with respect to the corresponding pixel gradient (line 1). 
% Each primitive is associated with several trainable parameters $x1, x2, x3, ...$. 
Each thread iterates through a list of its associated primitives (line 2, 3). Several intermediate conditions (like $cond1, cond2, ..$ shown in lines $5$ and $9$) determine if the current thread should contribute to the current primitive's gradients. Each thread then computes the gradient contribution of the primitive's parameters ($grad_t x1, grad_t x2, ...$). Finally, each thread performs an atomic add operation to accumulate its gradient contributions to the primitive's parameters (shown in lines 12-14). 
% There are several conditional branches that lead to thread divergence. This typically lead to only a subset of the threads performing the atomic operations.

\begin{figure}[!htb]

 \colorbox[RGB]{239,240,241}{
     \begin{minipage}{.9\linewidth}
\begin{algorithmic}[1]

\Function{BwdShaderKernel}{prims\_per\_thread}

\State $tid \gets thread\_idx$
\Comment{Thread corr. to pixel}
\For{ $p : primitives[tid]$ }
\Comment{Iterate}
\If{ \Call{cond1}{} } 
    \State \textbf{continue;}
    \Comment{thread doesn't participate}
\EndIf
    \State ...    
\If{ \Call{cond2}{} }
    \State \textbf{continue;}
    \Comment{thread doesn't participate}
\EndIf

    \State ...    
    \State ...    
\Comment{Gradient computation is done here}
    \State ...    

    \State \Call{AtomicAdd}{$p.grad\_x1$,  $\nabla^{tid}_{x1} $}
    \State \Call{AtomicAdd}{$p.grad\_x2$,  $grad_t x2$}
    \State \Call{AtomicAdd}{$p.grad\_x3$,  $grad_t x3$}
    \State ...    

\EndFor

\EndFunction
\end{algorithmic}
\end{minipage}
}

\caption{Outline of the shader's backward pass} 
\label{fig:atomicimplementation}
\end{figure}


% \todo{merge with previous, half this size, remove glue sentences. don't confuse fig. with algorithm}
% \subsection{Volume of Atomic Operations Made, and Atomic Reduction Bottleneck}

% As each thread of the shader's backward pass kernel corresponds to a single pixel of the rendered image,
% A high resolution image would fully occupy all the SM cores on the GPU. 
From Alg.~\ref{fig:atomicimplementation}, we make the observation that each thread iterates through a number of geometric primitives, and each loop iteration updates a set of parameters of the corresponding primitive. 
This means that a massive number atomic operations are sent each iteration (in the order of a few 10s to 100s of millions). These atomic operations lead to: 
\textbf{(1)} Oversubscription of atomic requests at the LSU instruction queue in each sub-core. \textbf{(2)} Contention in processing of atomic requests at the ROP units. 
To evaluate the effect of this, we perform an experiment to measure the percentage of stalls caused by contention of the LSU. We demonstrate our results in Fig.~\ref{fig:atomics_bottleneck}.  Across various differentiable rendering workloads (see Section~\ref{sec:methodology}), we observe a large percentage of stalls caused by LSU contention.

%This leads to a significant bottleneck in executing atomic parameter reductions at the L2 level.
%Executing these requires a long latency, as processing atomic operations requires an acquire and release operation to be performed along with a floating point addition. 

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/temp/perc_atom_stalls.png}
    \caption{Percentage of stalls resulting from execution of atomic operations}
    \label{fig:atomics_bottleneck}
\end{figure}

% Throttling of the L1 load requests (where atomics requests are sent)
% This is because of there are only a few 100s of ROP units in the memory partitions that process these atomics requests ( Section~\ref{sec:bckg_atomicprocessing}).


We also observe that the NVIDIA RTX 4090 GPU has a larger percentage of stalls in issuing instructions to the LSU instruction queue when compared against NVIDIA RTX 3060.
This is because more recent GPUs have higher shader compute compared to ROP compute. In our experiment setup, the NVIDIA RTX 4090 GPU has 4x more SM cores compare to NVIDIA RTX 3060 GPU (144 SM cores and 28 SM cores respectively). However, the RTX 4090 GPU only has about 2.5x more ROP units available (196 ROP units and 86 ROP units respectively).
% GPUs that pack a large number SM compute cores compared to the ROP units lead to a bottleneck in processing atomic operations, as the shader-core computation component is diminished with respect to that computed at ROP. 





\subsection{Key Observations}
\label{sec:motivation_observations}
We make the following observations from profiling atomic operations in the backward pass. 
\subsubsection{Observation 1} \textbf{Large degree of common parameters performed by atomic updates by the threads of the warp.}
Each primitive affects a region of pixels on the screen, known as a "fragment" (Section~\ref{sec:bckg_diffrendering}). As a result, close-by pixels that belong to the same fragment update the same primitive.  
% Each thread of the backward shader kernel iterates through a list of geometric primitives and updates its parameters (from algorithm~\ref{fig:atomicimplementation}).
Fig.~\ref{fig:raster_locality_schematic} shows how adjacent/close by pixels are part of the same fragment during rasterization. Fig.~\ref{fig:raster_locality} shows a geometric primitive in space \circled{1} rasterized onto a screen \circled{2} as seen from the camera indicated by the blue pixels during rendering. In the backward pass, each of these blue pixels affected is going to update the geometric primitive. A zoomed in version of the captured image is shown in Fig.~\ref{fig:zoomed}. We see that a single primitive rasterized onto a set of pixel leads to nearby by pixels being updated by the same primitive. 


\begin{figure}[!htb]

    \begin{subfigure}{0.27\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/motivation_rast.png}
    \caption{Close-by pixels are likely to be influenced by same geometric primitive.}
    \label{fig:raster_locality}
    \end{subfigure}~
    \begin{subfigure}{0.225\textwidth}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/motivation_imgbwd.png}
    \caption{Backward pass updates gradients w.r.t affected geometric primitive for each pixel}
    \label{fig:zoomed}        
    \end{subfigure}
    \caption{Close by threads update the parameters of the same primitives, on fragments produced by rasterization.}
    \label{fig:raster_locality_schematic}        

\end{figure}

This implies that threads within a warp, which correspond to a local region of pixels, compute the gradient component of the same primitive. 
These gradient components are then atomically summed up across threads to produce the parameter's gradient.
We perform an experiment to find the distribution of the number of threads in each active warp that atomically update the same primitive's parameters (and thus the same set of parameters). Fig.~\ref{fig:atomics_locality} shows a histogram of the total number of distinct primitive whose parameters are updated by each warp  (at each loop iteration of Algorithm~\ref{fig:atomicimplementation}). We observe that a large portion of threads in each warp update the gradients of the same primitive.  

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/temp/distinct_warp_atom_prim.png}
    \caption{Number of distinct primitives across 32 threads in a warp. 1 distinct primitive implies that all active threads in the same warp share the same primitive value, thus their atomic updates will target the same memory address determined by this shared primitive.}
    \label{fig:atomics_locality}
\end{figure}


\subsubsection{Observation 2} 
\textbf{Only a fraction of the threads within a warp perform atomic updates.}
% not issuing atomic requests for gradient update
From algorithm~\ref{fig:atomicimplementation}, we see that shader's backward pass has certain dynamically determined conditions ($cond1, cond2, ...$), that cause some threads to skip the current iteration of gradient updates. This implies that only a fraction of all threads send out atomic request within each warp.
%Which thread participates in the atomic reduction is dynamically determined based on the runtime information of the application.
We measure the number of threads that participate in the atomic reduction in 
Fig.~\ref{fig:atomics_unconvergent_warp_instructions}, for two different datasets (refer to Section~\ref{sec:methodology} for workload-dataset configurations). We observe that a varying fraction of threads within a warp produce atomic updates to global memory. 

\begin{figure}[!htb]
\begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/temp/hist_active_warp_thd_3dgs_playroom.png}
    \caption{Experiment on 3DGS Playroom}
    \label{fig:atomics_unconvergent_warp_instructions}
\end{subfigure}

\begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/temp/hist_active_warp_thd_nvdiff_lego.png}
    \caption{Experiment on NvDiff Lego.}
    \label{fig:atomics_unconvergent_warp_instructions}
\end{subfigure}

    \caption{Number of threads participating in atomic reduction.}
\end{figure}


\todo{insert the goal here - and talk about prior approaches}
Our \textbf{goal} in this work is to accelerate raster-based differentiable rendering applications by accelerating the processing of atomic reduction operations which constitutes a significant bottleneck in these applications. 





% \todo{connection to motivate our appraohc}
% \subsection{Existing Approaches that Use SM Level Reduction}


% Existing CUDA libraries and software frameworks~\cite{warplvlredcuda, cccl} can leverage unique property 1 to do warp-level or block-level reductions in the SM core, and then send a single atomic add instruction with the computed sum. However, this requires all threads within a warp to be active, and an additional check to be performed for all addresses to be the same, which may not necessarily be the case. Prior HW approaches~\cite{dab,lab} can leverage the property that several atomics update the same address by doing an warp level reduction. However, as only a fraction of the threads are active, the additional control flow latency introduced in doing an SM-level reduction will lead to buildup of a bottleneck in the SM core. This results in the shift in the atomic bottleneck from the memory partition to SM. This may not be optimal, as the ROPs in memory partitions are now underutilized. Hence, to address this problem, our  approach appropriately distributes the reduction computation work between the SM and the core.









==> text_srcs_old/abstract.tex <==
Graphics Processing Units have most widely been 






==> text_srcs_old/approach.tex <==
We introduce \projname, a primitive that enables fast atomic operation reduction when in applications when \textbf{(1)} several threads of a warp perform aggregation of a set of parameters corresponding to the same primitive, and 
\textbf{(2)} Only a fraction of the threads participate in performing atomic reduction.
The key idea of \projname is to (i) aggregate the common parameters' reduction computation at the sub-core level, and (ii) to 
We present two implementations of the primitive \projname: SW and HW implementation of this primitive. Our SW architecture design that selectively performs atomic operation reduction at the sub-core level to eliminate the atomic update bottleneck. \projname appropriately schedules reduction at the sub-core level as well as at the ROPs, based on the contention of resources at each unit.
% level atomic aggregation scene-parameter gradient computation in raster-based inverse rendering applications that have several threads computing the gradient of parameterized geometric primitives constituting the scene. These gradient components are then summed up (reduced) with atomic operations to produce the final gradient. 

% ADR edit: leverage the fact that several threads within a warp compute the gradient components of the same primitive to perform opportunistic aggregation and reduce the total number of atomic requests sent by each sub-core




%this sounds the same as point i?
A key challenge in distributing the computation across the SM core and the memory partition is managing the contention of compute resources at the L2 partition and the SM core. For instance, performing the entire reduction operation on a particular parameter in the SM core leads to a compute bottleneck on the FP units, leaving the ROP units at the L2 partition (where atomic operations are processed) idle, and vice versa.
To address this, we first outline our SW approach that computes a part of the reduction operation within the SM, and a part at the L2 unit. We describe how we can control the "amount" of reduction summation computation that is to be done at the SM vs the interconnect using a tunable hyperparameter.
We can then tune this hyperparameter to reduce the amount of idle time of the L2 ROP units and the FP units at the core.
% This parameter controls the ratio between warps that send atomics directly to L2 and warps that perform reduction.
\todo{maybe we mention interleaving?}

This approach, however, requires a significant engineering effort by the programmer and careful tuning in distributing this reduction computation. It also incurs additional overhead in performing branching instructions, leading to a slowdown \todo{diminished speedup}. To address this, we introduce \projname, a hardware mechanism that (i) adaptively tunes and manages the reduction  computation done at the L2 ROPs\todo{L2 ROP handle single atomic reqs} and the SM core (ii) requires no change in interface to the programmer (iii) eliminates the need for control flow instructions and redundant computation inevitable in SW, making it more power efficient\todo{making it faster?}. 

A high-level view of \projname is shown in Fig.~\ref{fig:distribution_reduction_high_level}. The reduction computation is completely performed in the SM core. The amount of reduction computation is adaptively controlled so that each resource is not kept idle.
% I think we should describe it as adaptively perform reduction when L2 ROP is occupied

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{figs/figure12.pdf}
    \caption{High-level overview of \projname}
    \label{fig:distribution_reduction_high_level}
\end{figure}


\subsection{Reduction Computation in the SM core}
% \begin{itemize}
%     \item Describe how reduction computation can be distributed
%     \item Provide mathematical equation for the reduction computation split
%     \item Describe what determines how much bottleneck is developed at each componetn - number of active threads doing the atomics overall - 
%     \item Mention that this depends on device, on application and dynamic parameters 
%     \item Describe our application profile.
% \end{itemize}
As described in Section~\ref{sec:motivation_shaderbwdimpl}, each thread in the backward pass of the shader kernel computes a \todo{set of components?} component of the gradient of a parameter $x_i$ corresponding to a primitive $p$ , which we denote as $grad_t\_x_i$. The gradient of a parameter $x_i$ (denoted as $grad\_x_i$ ) of primitive $p$ is computed as a reduction (summation) of the gradient components computed by each thread as follows:
\begin{equation}
    p.grad\_xi = \sum_{t\in \mathcal{P}} p.grad_t\_xi
\end{equation}
Where $\mathcal{P}$ is the set of threads updating the gradient of parameters of the primitive $p$.
Each thread computes one term of this summation, and these terms are summed up to produce the total gradient with an atomic add operation. 
However, this results in a significant amount of time spent in evaluating atomic operations  
% is this just atomic bottleneck?
(Section~\ref{sec:motivation_observations}).

As several threads of each warp (which correspond to close by pixels) compute the gradient of parameters of the same primitive, we can alleviate the bottleneck by summing up the gradient of common parameters at sub-core level first, and then use a single atomic add operation on the result of the summation.
Within each warp, the threads summing to the same parameter can first be summed up at warp level as expressed below below:
\begin{equation}
    \label{eq:warpred}
    p.grad\_xi = \sum_{w\in \mathcal{W}} \sum_{t\in w(\mathcal{P})} p.grad_t\_xi
\end{equation}
where $\mathcal{W}$ is the set of all warps, and $w(\mathcal{P})$ is the set of threads in the warp updating the parameter $p$. The inner summation in Eq.~\ref{eq:warpred} can be computed within a single SM, using warp level primitives.

However, doing the reduction computation in the SM incurs an additional cost in control flow in finding the set of threads that update the same parameter before summing them. This adds a significant latency in evaluation of the atomic operation. We find that the cost of doing this might become significant bottleneck, and we show that it will ultimately slow up the application (Section~\ref{sec:results}).
% or maybe doing reduction trivially will slowdown the application

\subsection{SW approach}
\label{sec:approach_sw}
\todo{Would it be a better flow if we introduce SW-S first, then we identify the reasons for diminished speedup, }
\subsubsection{Controlling the Amount of Reduction Computation in SM vs L2 ROP units}

We need to ensure that the number of cycles spent in performing the reduction operation is the least it can be, before it becomes the main bottleneck. A reasonable method to modelling the latency required to the reduction at the SM-level is to count the number of floating point numbers that are required be summed up. We call this count, the "active count". 
This count is used to approximately model the latency of the reduction operation, as the active count parameter is monotonically related to the latency to compute the summation in the sub-core. Based on this "active count", we determine the appropriate location to do the warp level computation (the inner computation). Fig~\ref{fig:balance_threshold} demonstrates how the number of active threads leads to different latencies in doing reduction in each thread <todo>.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.5\linewidth]{example-image}
%     \caption{Microbenchmark of SM reduction latency with different active counts, vs ROP reduction latencies \todo{we're planning to remove this}}
%     \label{fig:balance_threshold}
% \end{figure}

We apply a threshold on this parameter to determine the appropriate location for doing the reduction.
We call this parameter the "balancing threshold", as it control the decision to doing reduction computation either in the SM core or the atomic units at the L2. Increasing the balancing threshold would lead to the longer latency reduction computation to be performed in the SM core while simultaneously freeing the bottleneck in the ROP units, and vice-versa. \todo{this is not true. Increasing balance threshold decreases overall number of reductions performed and increases total number of atomics sent to L2.}

\subsubsection{Factors influencing bottleneck in reduction computation}
The appropriate balancing threshold parameter depends on the level of contention of the L2 ROP units, as well as latency in doing reduction at the SM core. This is influenced by the amount of reduction operations to be performed, which in-turn depends on several factors, outlined below: 
\begin{itemize}
    \item \textbf{Dataset and workload type:} The amount of reduction computation to be done depends on the workload (scene representation primitives, camera resolution, etc.) and the scene data it's learning (detailed, large scale scenes with several primitives are slower to learn).
    % Different characteristics


% \begin{table}[!htb]
%     \centering
%     \begin{tabular}{c|c|c|c}
%         \textbf{Workload}     & \textbf{Atomic} & \textbf{Arithmetic} & \textbf{Best} \\
%         \textbf{}     & \textbf{Intensity} & \textbf{Intensity} & \textbf{Method} \\
% \hline
%         \texttt{gsplat}     & med  &  &  balanced   \\
%         \texttt{nvdiffrec}  & low  &  &  SM-reduce   \\ 
%         \texttt{pulsar}     & high &  &  serial-SM-reduce   \\

% \end{tabular}
%     \caption{Characterization of atomic intensity and arithmetic intensity of the workloads base don profile}
%     \label{tab:characterization_of_workload_and_method}
% \end{table}

    
    \item \textbf{GPU device architecture:} The different compute throughput of the GPU's SM cores vs the L2 ROP units influences the speed with which reduction computation that can performed. We test our approach on two different configurations: one with an RTX 3060 GPU configuration (low SM count compared to ROP units) and an NVIDIA RTX 4090 GPU (high SM count comprated to ROP units).
    
    \item \textbf{Reduction method used:}  Different methods of parallelizing the SM level reduction leads to different speedups, with a different set of trade-offs. In this work, we present two methods to do reduction in software, described below. 
\end{itemize}

% \subsubsection{\projname in Software}

% \begin{itemize}
%     \item Computation required to do reduction computation - mention what it depends on : check for common address for several atomic parameters
%     \item describe how this check can be done <once> - leading to speedup
%     \item Reduction can be performed in two ways - butterfly reduction and serialized reduciton, each with it's own tradeoffs and core contention profile.
% \end{itemize}


\subsubsection{\projname Serialized Execution}
% we hsould mention that this is a more general solution that do not require full convergence? Maybe we talk about butterfly first?
This approach requires looping through the computation of each operation.
The latency to do summation in this manner is proportional to the number of gradient parameters to be added. This approach however, is inefficient as a number of the summations can be parallelized. This incurs significant reduction in atomic latency as ...
A schematic of our software approach is shown in Fig.~\ref{fig:serialized_overview}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=.76\linewidth]{figs/figure14.pdf}
    \caption{Serialized reduction implementation overview}
    \label{fig:serialized_overview}
\end{figure}

\subsubsection{\projname butterfly reduction}
Fig.~\ref{fig:bfly_overview} shows an overview of the schematic used in the butterfly reduction. In this approach, we first check whether all the threads of the warp update the same primitive. If so, we use a reduction tree to compute the summation of each parameter.
This approach, however, requires all threads to be kept active. This means that the threads were originally inactive are required to sum an additional 0 value for the implementation.   
% This implies the programmer has to enforce convergence by keeping all threads alive and assigning 0-value gradients to threads that do not participate in the gradient update.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=.75\linewidth]{figs/figure15.pdf}
    \caption{Reduction-tree / butterfly reduction implementation overview}
    \label{fig:bfly_overview}
\end{figure}


\subsection{\projname - Hardware Design}
\label{sec:approach_hwdesign}

Our software approach has several limitations in executing a warp level primitive operations outlined as follows: 
% i is only true for SW-B. maybe we should talk about ii iii and iv as i ii iii and then mention i as an additional overhead for SW-Bs
(i) Incurs additional overhead in performing redundant computations in doing the reduction operation at the warp level, as only a fraction of all threads are producing actual updates every iteration. (ii) Introduces overhead with control flow instructions per thread in trying to do warp-level reduction (iii) Requires significant programmer and engineering effort in using warp level primitive instruction (iv) Requires careful tuning of workload and device-dependent hyperparameter to get the best-case speedup.

In order to address these issues, we introduce \projname, a sub-core level microarchitecture design to efficiently process the reduction summation operations for GPUs. \projname first finds groups of atomic instructions that update the same memory location by active threads in the warp. It then adaptively selects the appropriate hardware target (SM subcore or L2 ROP units) where summing-up operations are to be executed based on the level of contention, and schedules the reduction computation appropriately. If the L2 ROP units are selected, the reduce operations are directly scheduled in the same manner as atomic operations. If the SM subcore is selected, the gradient components from different threads re summed-up and the resulting sum is issued to L2 ROP units.
This ensures that the L2 ROP units are always kept busy during execution, while ensuring that it doesn't develop into contention.
% and lead to long stalls
Finally, in order to expose this functionality to the programmer, we encapsulate our sub-core reduction mechanism with a new warp-level instruction which we call "\atomred{}" instruction. Our modified GPU architecture schedules and decodes these \atomred instructions into one of the sub-cores.    
We implement our design by introducing three HW modules to the GPU sub-core microarchitecure to process these \atomred instructions: the \redcoalesce module, the contention determination module , and the \reduce module which picks up issued reduction operation. A high level overview of the design is shown in Fig.~\ref{fig:scar_high_level}.
% atomred is a seemingless swap from normal atomics
\begin{figure}[!htb]
    \centering
    \includegraphics[width=.75\linewidth]{figs/figure16.pdf}
    \caption{HW walkthrough of \projname \todo{this picture needs to change}}
    \label{fig:scar_high_level}
\end{figure}

\subsubsection{Atomic address coalescing}

The address coalescing module finds groups of active threads that point to the same memory address and coalesces them together to produce groups of \atomred request. This identification of common addresses is implemented using the same logic that is used to coalesce common memory addresses of all threads performing a load operation.

\subsubsection{Contention determination module (CD)}
The contention determination module receives reduction computation from the dispatch port (of each sub-core) of the load-store unit and checks whether. Is first checks whether the L2 interconnect queue is free to issue instructions into memory partition's ROP unit. If this queue is full, it  schedules the reduction operation to be processed by the reduction computation unit described below. 

\subsubsection{Reduction computation module}
The reduction computation unit contains a single floating point unit, which processes the summation computation of each group (coalesced unit) scheduled sum in a serial manner. 







==> text_srcs_old/background.tex <==
\noindent 

\subsection{Learning Scene Representations with Differentiable Rendering}

In several tasks such as 3D scene reconstruction and inverse rendering, the training pipelines typically involves producing an image from a parameterized scene representation, and comparing this with a ground truth image (as shown in Fig.~\ref{fig:inverse_rendering}). A loss function which measures the difference between the ground truth image and the rendered image is then computed.
This loss function is minimized by backpropagating the loss derivative to obtain the derivative with respect to the scene parameters, and then applying gradient descent on these parameters.
In order to do this, a differentiable renderer, which computes the loss derivative with respect to scene parameters is used.


\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/inv_render_intro.pdf}
    \caption{Common differentiable rendering optimization pipeline.}
    \label{fig:inverse_rendering}
\end{figure}


\subsection{Rasterization-and-shading based Rendering Pipeline}
\label{sec:bckg_diffrendering}
Traditional raster-based rendering pipelines (shown in Fig.~\ref{fig:rast_and_shading}) considers the scene being comprised of several fundamental geometric objects, or "primitives", in 3D space (such as a mesh composed of triangles, point cloud, spheres, etc.). These primitives are associated with rendering parameters (color/normal/material). These primitives are rendered as seen by a camera on screen using the rendering pipeline, consists of the pre-processing stage (primitive culling), rasterization, + shading, and blending. The rasterizing and shading stages are described below: 1) \textbf{rasterization}: involves finding the list of primitives that are going to affect each pixel (known as \emph{fragments}) of the rendered image, and 2) \textbf{shading}: involves determining the color of each fragment that is going to contribute to the color of each pixel in the rendered image.

\subsubsection{Differentiable Rendering on rasterization pipeline}

\emph{Differentiable} raster-based rendering pipeline adds a backward pass routine - referred to as the backward shading kernel which performs the sequence of steps depicted in Fig.~\ref{fig:backward_pass_renderer}. The routine receives as input a pixel-wise list of fragments (primitives which influence it's color) and loss gradient with respect to the fragment. 
This loss gradient with respect to the image is a large $H\times W\times C$ array, where $H, W, C$ correspond to the height, width (in number of pixels) and number of color channels of the image. Each element is the loss gradient with respect to the corresponding pixel's color channel. From each of these elements, it first computes the pixel's contribution of loss gradient w.r.t parameters of each primitive (corresponds to each fragment). It then aggregates these gradient contributions of all pixels for each primitive to produce the parameter gradient.
% Out of these stages, a vast amount of work in computer graphics literature over the years focused on optimizing the rasterization stage SW and shading stage~\cite{opengl}. The 

\begin{figure}[!htb]
    \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=0.85\linewidth, trim={5 0 0 0},clip]{figs/resterization_pipeline.pdf}
    \caption{Traditional rasterization based rendering pipeline}
    \label{fig:rast_and_shading}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
    \vspace{10pt}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/resterization_pipeline_bwd.pdf}
    \caption{Backward pass of the raster-based rendering pipeline}
    \label{fig:backward_pass_renderer}
    \end{subfigure}
    \caption{Forward and backward pass of the differentiable rendering pipeline}
\end{figure}

\subsection{Baseline GPU Architecture and Atomic Operations Processing}
\label{sec:bckg_atomicprocessing}
% Each programmed as a set of SIMD instructions, known as a warp intructions that produce L2 
Fig.~\ref{fig:sm_baseline} shows the schematic of a baseline architecture of the streaming multiprocessor (SM) in a modern GPU. Each SM of the GPU is composed of multiple sub-cores \circled{1} (typically 4, as shown in the figure) which handles instruction execution and a memory I/O (MIO) block \circled{2}, which handles memory transactions. Each sub-core consists of a register file, the instruction frontend \circled{4} (instruction cache,  warp scheduler, instruction decoding and operand collection logic), execution units \circled{5}, and load store (LDST) units \circled{6}. The MIO block consists of the L1 data cache, shared memory space and the load-store queue (LSU)\circled{3}.

Atomic instructions dispatched by the frontend \circled{4} are received at the LDST unit of the sub-core\circled{4}. The LDST unit produces a memory transaction for atomic request called by each active threads in the warp, and enqueues them to the instruction queue to the LSU unit in the MIO block \circled{3}. The LSU unit receives these request and issues them to the memory partition where the atomic requrests are processed. The memory partition interfaces the L2 and global memory, and consists of render operation units (ROP)\circled{7}. These ROP units consist of floating point hardware that atomically computation and writes updates the atomic request's address to L2.  


\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{figs/bckg_gpu.drawio.pdf}
    \caption{Baseline model of a single GPU's SM Architecure}
    \label{fig:sm_baseline}
\end{figure}


% \subsubsection{Renderer Backward Pass}
% \label{sec:background_shaderbwdimpl}
% % \subsection{Implementation outline of the backward shader kernel}

% % Here, we inspect the backward shader kernel in further detail. \todo{is this professional?}
% The input to the backward pass is a set of per-pixel lists of primitives that influences the color of the corresponding pixel (discussed in Section~\ref{sec:bckg_diffrendering}). The backward pass iterates through this list of primitives to compute the gradients of each primitive for each pixel. This is an embarrassingly parallel computation that is trivially parallelized across pixels, with each thread performing the computation for one pixel. The gradient computation in the backward pass of differentiable rendering workloads is depicted in Alg.~\ref{fig:atomicimplementation}. 
% % the gradient of a loss function with respect to parameters of scene primitives, from the gradient loss with respect to the pixel color channels.
% % Each thread receives a list of primitives as input and computes the gradients of the parameters of each primitive with respect to the corresponding pixel gradient (line 1). 
% % Each primitive is associated with several trainable parameters $x1, x2, x3, ...$. 
% Each thread iterates through a list of its associated primitives (line 2, 3). Several intermediate conditions (like $cond1, cond2, ..$ shown in lines $5$ and $9$) determine if the current thread should contribute to the current primitive's gradients. Each thread then computes the gradient contribution of the primitive's parameters ($grad_t x1, grad_t x2, ...$). Finally, each thread performs an atomic add operation to accumulate its gradient contributions to the primitive's parameters (shown in lines 12-14). 
% % There are several conditional branches that lead to thread divergence. This typically lead to only a subset of the threads performing the atomic operations.

% \begin{figure}[!htb]

%  \colorbox[RGB]{239,240,241}{
%      \begin{minipage}{.9\linewidth}
% \begin{algorithmic}[1]

% \Function{algorithm}{prims\_per\_thread}

% \State $tid \gets thread\_idx$
% \Comment{Thread corr. to pixel}
% \For{ $p : primitives[tid]$ }
% \Comment{Iterate}
% \If{ \Call{cond1}{} } 
%     \State \textbf{continue;}
%     \Comment{thread doesn't participate}
% \EndIf
%     \State ...    
% \If{ \Call{cond2}{} }
%     \State \textbf{continue;}
%     \Comment{thread doesn't participate}
% \EndIf

%     \State ...    
%     \State ...    
% \Comment{Gradient computation is done here}
%     \State ...    

%     \State \Call{AtomicAdd}{$p.grad\_x1$,  $\nabla^{tid}_{x1} $}
%     \State \Call{AtomicAdd}{$p.grad\_x2$,  $grad_t x2$}
%     \State \Call{AtomicAdd}{$p.grad\_x3$,  $grad_t x3$}
%     \State ...    

% \EndFor

% \EndFunction
% \end{algorithmic}
% \end{minipage}
% }

% \caption{Outline of the shader's backward pass} 
% \label{fig:atomicimplementation}
% \end{figure}




% \subsubsection{GPU Memory consistency model in relation to atomic operations processing}

% The PTX instruction set, an intermediate representation instruction set used in NVIDIA GPUs, provides well defined semantics to express the memory consistency model, specified by the instruction set documentation~\cite{ptxisa, formalptxmc}. Most GPUs implement a version of Heterogeneous race-free for sequential consistency (HRF-for-SC) model. This model defines memory consistency across various scopes of memory, specifying memory ordering constraints for different memory regions visible to the programmer. Local and global scope~\cite{}. In this work, we are concerned with the accesses made by the memory mode ltowards the global scope This model provides semantics  by a store-release
% Shared weight parameters of the thread can be made via  memory operations 

% GPU memory consistency models is defined at scopes, for . The consistency model for \texttt{atom} and \texttt{red} instructions  is specified by 


% The memory consitency model provideds Load-acquire and store-release semantics


% The atomic operations of the GPU are processed at the memory partition which indexes a sereies of the L2 cache.  




==> text_srcs_old/detailed_design.tex <==
\label{sec:design_main}

In this section, we describe each component defined of our design constituting of SW component and a HW component

\subsection{SW approach in reduction execution balancing split}

\subsection{\redcoalesce module}
\label{sec:design_redcoalesce}




\subsection{\reduce module}
\label{sec:design_reduce}



\subsection{\reduce vs Atomic load policy}
\label{sec:design_reduce}
The total amount of reduction parameters used for the total


\subsection{Overheads Analysis}
\label{sec:overehads_analysis}


\subsection{Analysis: Feasibility of design}


\textbf{latency store overheads}





==> text_srcs_old/introduction.tex <==


\todo{improve the first sentence - deleted}
\todo{start with.... inverse rendering is an important problem ... }
% Graphics processing units (GPUs) trace their inception as an accelerator to render a 3D scene containing several objects in it into an image to be displayed on screen.

\todo{something - along the lines of - atomics have been studied for a long time ;;;;; position half the paper  }

\todo{Say there's a huge amount of interest with these applications}

Inverse rendering is a fundamental and an important problem in computer graphics, which involves deriving properties of the 3D environment (such as geometries of objects, color, material properties, etc.) from a set of images captured by cameras overlooking the scene.
These scene representations are used in several current and upcoming applications, such as photogrammetry, 3D modelling and scanning, 3D model creation tools, game engines, AR/VR applications, etc. 
As a result of recent interest in inverse rendering, there is a growing trend to incorporate their support in GPUs as a first class feature~\cite{slang}. 

\todo{Say there's a huge amount of interest}
Recent works have demonstrated success applying gradient-based optimization techniques to inverse rendering problems~\cite{3dgs, pulsar, nvdiffrec, dmtet, flexicubes, instantngp, dvgo, plenoxels, nerf, neus}. GPUs are widely used as the prim. \todo{complete}

\todo{One line of work uses nerf research. Compared to those, thsese appraches have emerged as being faster}


\todo{A recent transformative work has spurred a lot of interest...}
For example, a recent and notable work in doing state-of-the-art 3D scene reconstruction in a fast manner is 3D Gaussian Splatting~\cite{3dgs}. This method has already been adopted in Unreal Engine~\cite{unreal}, a mature 3D modelling application / game engine. It is used in obtaining a 3D model of real-world.

% Inverse rendering involves learning a parameterized scene representation by minimizing the loss between an image rendered using this scene parameters and a ground truth image. 
% This loss function is minimized using gradient descent, which uses a differentiable renderer to compute the gradient with respect to scene parameters.
% A typical parameterized scene representation considers the scene being comprised of several fundamental geometric objects, or "primitives", in 3D space (such as a mesh composed of triangles, point cloud, spheres, etc.), each one associated with material properties (reflectance/color/texture). These primitives are rendered as seen by a camera using the rendering pipeline, which consists of 2 main stages: 1) \textbf{rasterization}: to find the list of primitives that are going to affect each pixel of the rendered image, and 2) \textbf{shading} - to determine the color each pixel in the rendered image by blending the radiance component of each primitive.
% \emph{Differentiable} raster-based rendering pipeline adds two additional routines: 1) backward rasterization - which is functionally similar to rasterization, and 2) backward shading: which takes as input the derivative of a loss function with respect to each of the pixel's color channel and computes the gradient of the parameters defining each primitive's location, shape and texture with respect to a loss function.
% Out of these stages, a vast amount of work in computer graphics literature over the years focused on optimizing the rasterization stage SW~\cite{opengl, tiled_rasterization, zbuffering} and shading stage~\cite{texturemem}.


Inverse rendering involves learning a parameterized scene representation by minimizing the loss between an image rendered using this scene parameters and a ground truth image. 
This loss function is minimized using gradient descent, which uses a differentiable renderer to compute the gradient with respect to scene parameters.
A typical parameterized scene representation considers the scene being comprised of several fundamental geometric objects, or "primitives", in 3D space (such as a mesh composed of triangles, point cloud, spheres, etc.), each one associated with material properties (reflectance/color/texture). These primitives are rendered as seen by a camera using the rendering pipeline, which consists of 2 main stages: 1) \textbf{rasterization}: to find the list of primitives that are going to affect each pixel of the rendered image, and 2) \textbf{shading} - to determine the color each pixel in the rendered image by blending the radiance component of each primitive.
\emph{Differentiable} raster-based rendering pipeline adds two additional routines: 1) backward rasterization - which is functionally similar to rasterization, and 2) backward shading: which takes as input the derivative of a loss function with respect to each of the pixel's color channel and computes the gradient of the parameters defining each primitive's location, shape and texture with respect to a loss function.
Out of these stages, a vast amount of work in computer graphics literature over the years focused on optimizing the rasterization stage SW~\cite{opengl, tiled_rasterization, zbuffering} and shading stage~\cite{texturemem}.

\todo{merge with shortened previous description}
The backward-pass of shader routine, however, constitutes a significant bottleneck in the overall rendering pipeline.
This routine takes up as much as 30-70\%\todo{check} of the overall runtime. 
Both the forward pass and backward pass of the shader routine consist of embarrassingly parallel computation. The forward pass has each thread independently compute the color of each pixel. The backward pass computes the gradient contribution of each primitive affecting each pixel. 
However, unlike the shader's forward pass, the backward-pass requires summing up (reducing) the contribution of the gradient computed by each thread, for each parameter.  
% This fundamentally requires communication across threads in updating the gradient parameter, requiring the need for synchronization routine between them. 
These computed gradients are summed up using atomic add operations in each thread.
Each primitive has several trainable parameters.
The number of atomic requests grows rapidly with image size (proportional to the number of pixels / quadratically with the resolution), and linearly with number of primitives contributing to the color of a pixel. 
This number can be as high as several tens of millions of operations for a high resolution image. 
Based on our profiling results, we observe that atomic operations constitute the primary bottleneck in the shader's backward pass.
This bottleneck arises because of overwhelming the ROP units (render operation units) in the memory partition, which execute atomic operations.

Prior work does SM level reduction ......
LG - Throttle
\todo{threads send too many atomics that throttles the L1 controller, causing stalls. }  This is because each pixel is associated with a large number of primitives, each primitive has many atomics ....
problem with workload


On analyzing the nature of the atomic operations launched during the shader's backward pass, we make the following key observations: 

\textbf{(1)} \todo{threads send too many atomics that throttles the L1 controller, causing stalls. }  This is because each pixel is associated with a large number of primitives, each primitive has many atomics .... 
\textbf{(2) \todo{Threads in a warp typically update the same parameter}. Common addresses in atomic operations within a warp:} A large number of threads of each warp do gradient updates to the same memory address via atomics. In fact, we find that the number of warps having all threads updating the same addresses are up to 95\%. This happens because the threads of a warp correspond to close-by pixels of the image, and the accumulate gradients of each primitive and each primitive influences affect a local set of pixels. 


\textbf{(2) Each primitive is associated with multiple trainable parameters:} Each primitive is associated with several trainable parameters. Updating each parameter requires a unique atomic request. Each of these atomic acquires a lock on memory locations corresponding to each of these parameters. However, all atomic gradient updates of parameters of a single primitive can instead be updated by acquiring a lock on a single index corresponding to the primitive being updated, \textbf{(3) Presence of inactive threads that do not produce atomic updates:} only a fraction of the threads in each warp send out atomic requests for gradient updates. We call these threads \emph{effectual} threads. The remaining fraction of threads enter a branch of execution that do not send out atomic requests (\emph{ineffectual} threads). Whether a thread is effectual or not is determined dynamically by the backward pass algorithm.  

To alleviate the atomic bottleneck, one possible approach is to leverage the fact that common addresses are updated by atomic requests to first to sum up all gradients contribution by threads within a warp / SM-level first. The result can then be sent out using a single atomic request. However, we observe that doing this in software will introduce a significant number of instructions and control flow, which can slow down execution significantly. 
Prior hardware approaches, such as atomic buffering (LAB~\cite{lab} and DAB~\cite{dab}), propose a technique to fuse atomic requests of each warp on atomics updating the same address dynamically by coalescing and computing the sum in each SM. However, doing complete reduction would lead to development of a new bottleneck from atomic requests at L2 to compute intensity in the core in doing reduction. 


\todo{develop a new method to address atomic problems of these types ..., such as the ones seen }

\todo{split goal and approach into different pararaphs}

\todo{A technique to do fast aggregation of gradient parameter}
Our \textbf{goal} in this work is enable fast execution of the parameter gradient update step of the shader's backward pass routine, which is useful to speedup several inverse rendering applications. To this end, we introduce \projname, a mechanism that enables fast computation of the gradients of scene parameters in raster-based inverse rendering pipelines. The key idea of \projname is to leverage the fact that several threads within each warp update the same gradient parameter, to express part of the gradient summation to be performed at each SM core, and a part to be done in the L2 ROP units such that are not kept starved from processing. 
The gradient parameter reduction work can then be scheduled either in the SM core, or the L2 ROP units, depending on the level of contention of hardware resources.   
Hence, we propose \textbf{(1)} A software approach that selects and schedules the computation of atomic reduction processing either in the SM core or the L2 ROP units based on the level of contention of each hardware resource. This approach performs a reduction at the SM-core level using warp level primitives (such as\emph{\_\_shfl\_sync}) to access thread data from different warps and then aggregating them using FP unit (+ operation). As each thread has to update several parameter of the primitive, this requires a check across warps to find the common address for each parameter. To alleviate this checks in doing reduction, the single primitive index for aggregation. 
A key challenge in this approach is determining the level of contention in the SM core and the L2 ROP partition, and managing while introducing minimal overhead at runtime. To address this, we introduce a hyperparameter which determines the number of summations to be performed in the SM core for doing reduction compared to the computation offloaded to the L2 ROP units. 

However, this approach requires hyperparameter tuning and a significant programming effort in implementing this solution. Additionally, the additional code introduced to do reduction at the SM-core level introduces additional control flow and compute latency overhead which could slow down the application.  
\textbf{(2)} In order to solve this, we propose \projname-HW solution, a HW mechanism that adaptively determines which parameters can be summed up at the SM level for doing reduction, and adaptively schedules the overall reduction computation to either the SM core or the L2 partition based on the level of contention of these HW resources. 

We evaluate our approach across recent notable inverse rendering workloads. With our SW appraoch, we achieve a speedup of up to \todo{}$\times$ on the backward shader kernel alone, and up to \todo{}$times$ overall application speedup. With \projname-HW, we achieve a speedup of up to \todo{}$\times$ on the shader kernel, and an upto  $\times$ overall speedup. Our list of contributions are summarized as follows: 
    \begin{itemize}
        \item We provide a detailed characterization of rasterization + shading based on a wide range of inverse rendering workloads
        \item Design our software approach to alleviate the bottlenck associated with reduction operations in computating the backward pass gradients, by
        \item Design \projname-HW, a HW mechanism that adaptively chooses reduction operation based on the level of contention of resources at the ROP units and the SM core.

    \end{itemize}








==> text_srcs_old/introduction_1.tex <==



Inverse rendering is a fundamental problem in computer graphics, which involves deriving properties of the 3D environment (such as geometries of objects, color, and material properties) from a set of images overlooking the scene.
These scene representations are used in several current and upcoming applications, such as photogrammetry, 3D modeling and scanning, 3D model creation tools, game engines, and AR/VR applications. 
There has been a huge level of interest in inverse rendering after recent works have demonstrated significant improvements in achieving high quality scene reconstructions as a result of incorporating learning based methods. i.e, Neural Radiance Fields, 3D gaussian splatting~\cite{nerf, 3dgs}.   
This success lead to recent work~\cite{slang}\todo{cite all slang works} proposing native support for inverse rendering in GPUs as a first-class feature. 

One approach to do inverse rendering is to use volumetric rendering~\cite{volume_rendering} for producing the scene that is represented using a radiance field~\cite{dvgo, plenoxels, instantngp, nerf}. Another approach is to use a fast and efficient raster-based rendering pipeline on a scene represented with a set of geometric \emph{primitives} in 3D space~\cite{3dgs, pulsar, nvdiffrec, dmtet, flexicubes, adop}. \todo{define primitive with example}
% These primitives constitute the 3D scene. 
In this work, we focus on raster-based inverse rendering pipelines.
% The radiance information in space is encoded using an MLP. Rendering an image This method requires computing and aggregating radiance information at several points in space to render a single image, leading to very slow training and rendering times. To address the slow training speeds, several algorithmic~\cite{dvgo, plenoxels, instantngp, mobilenerf} as well as hardware architectural solutions~\cite{neurex, instant3disca, gennerf, artist} have been proposed which brought down the learning time of a high-quality scene representation from a few days to a few minutes. However, achieving SOTA reconstruction is still comparatively slow.
% Using fast and efficient raster-based rendering pipeline on a scene represented with a set of geometric primitives in 3D space~\cite{3dgs, pulsar, nvdiffrec, dmtet, flexicubes, adop}.
A recent transformative work, 3D gaussian splatting~\cite{3dgs},  uses a high-speed rasterization pipeline for rendering. This has spurred tremendous interest in the computer graphics community and has demonstrated state of the art capability in producing high-accuracy, high-quality scene reconstructions at a very high speeds.
% when compared to volumetric rendering based approaches. 
It represents the scene geometry with 3D gaussians as its primitives, and associates each gaussians with a view-direction dependent color. It uses an efficient tile-based rasterizer~\cite{adop, pulsar} over the 3D gaussians which are then colored to produce an image of the scene.  
The sheer level of successes of this method lead to its adoption in Unreal Engine~\cite{unreal}, a mature 3D modelling application / game engine, where it is used to obtain a 3D model of the real-world.

\todo{differentiable rendering at the start - move this up front. Recently there has been sota mehtods in diff. rendering . Introduce nerf.}
These raster-based rendering methods learn the parameters of geometric primitives in the scene by first computing a loss between a rendered image and the corresponding ground truth image. 
This loss is minimized using gradient descent. To compute these gradients with respect to scene parameters, a \emph{differentiable} renderer is used.
A differentiable renderer computes the loss gradient w.r.t each primitive in the backward pass (referred to as \emph{backward shading}).
% It takes as input the loss gradient w.r.t to the image and computes the gradient w.r.t the each primitive's parameters.
Each thread of the backward shader kernel is associated with one pixel. It computes and then accumulates the gradient contribution of each primitive w.r.t its pixel color.
% These gradient contributions to each primitive are then accumulated using operations.
% that influences the color of \todo{or effecting the color of?} each pixel. 


This backward-pass of shader routine constitutes a significant bottleneck in the inverse rendering pipeline, taking up as much as 30-70\%\todo{check} of the overall time (see section~\ref{sec:motivation_backward_runtime}). 
We observe this bottleneck is primarily caused by the overwhelming number of atomic operations launched during gradient accumulation step. The atomic operations issued by the sub-cores are queued to the instruction queue leading to the LSU (Load-Store-Unit) that handles memory operations in the SM. 
This causes high contention at the LSU. (Section~\ref{sec:motivation_shaderbwdimpl})
% the \emph{ROP} units (stands for \emph{render operation units}, which execute atomic operations in the memory partition).
% The backward-pass requires summing up (reducing) the contribution of the gradient components with respect to the primitive's parameter computed by each thread.  
% These computed gradients are summed up using atomic add operations in each thread.
Prior approaches~\cite{lab, massiveatomics, acceleratingatomics} address bottlenecks due to atomic requests with SM-level reduction before sending them to the memory partition.  
This involves aggregating individual gradient components produced by each thread on the L1/shared memory.\todo{In these applications, it doesn't work because we see that the LSU is overhelemed ...}
% first, and then sending atomicallty adding the result of this summation. 
% To alleviate the control flow overhead in doing this in software, 
% These methods can alleviate the level of contention at the ROP units in the memory subpartition. 

However, aggregating gradients at the SM-level will not alleviate contention at the LSU, as atomic requests only arrive at L1/shared memory after it leaves the LSU. 
% This makes aggregating at the L1 level (SM-level) itself a significant bottleneck. 
% This contention at the LSU happens because the number of atomic sent is overwhelmingly high.

% This high-number of atomic operations is a consequence of these workloads rendering highly detailed scene into a high resolution image. The number of atomic requests grows rapidly with image size (proportional to the number of pixels / quadratically with the resolution), linearly with number of primitives contributing to the color of a pixel, and linearly with the number of parameters per primitive. 
% Hence, each pixel is associated with a large number of primitives, and each primitive has many parameters.
% In-effect, this leads to the number of atomic requests sent out to be as exceptionally high (as much as  several tens of millions of operations in a millisecond for a high resolution image).


On further analyzing the nature of the atomic operations launched during the shader's backward pass, we make the following key observation: threads in a warp typically update parameters of few distinct primitives. In fact, we find that the number of warps having all threads update the same primitive are up to 95\%. This leads to a large number of threads in a warp to add gradient updates to the same set of memory addresses via atomic requests. 
% This happens because the threads of a warp correspond to close-by pixels of the image, and the accumulate gradients of each primitive and each primitive influences affect a local set of pixels. 
% To alleviate the atomic request bottleneck, o
One approach that leverages this key observation to alleviate atomic request bottleneck is by summing up gradient contributions to the same parameter from all threads within a sub-core. This reduces the total number of atomic requests sent to the LSU at SM-level, which alleviates the LSU contention. The result can then be sent out using a single atomic request per sub-core, for each parameter. 
% As a warp executes within each sub-core, this set of operations can be performed in software. However, doing this in software this reduction techniques has to be performed for each individual parameter, requiring several checks and introduces a significant number of instructions and control flow, which can slow down execution significantly.

% Prior warp level reduction in
% However, we observe that doing this in software will introduce a significant number of instructions and control flow, which can slow down execution significantly. 

% \todo{Narrative: key idea of \projname-SW appraoch: grouping several parameters in reduction ocmputation to reduce control flow overhead. HTis introduces significant programmer overheaf + still has control flow instrucionts slowing it down. \projname-HW addresses this with native support for tha eliminates .

% A key challenge in doing this is that sub-core reduction might become a significant bottleneck in handling the reduction computation completely by itsefl. This would lead to development of a new bottleneck from atomic requests at L2 to compute intensity in the core in doing reduction.

% In SW- we solve this withballancign threshold parameter and modelling subcore latency with instruciton coutn. in HW - no tuning required and adaptively schedules reduction computation to either ROP or subcore based on level of contention.
% }

\todo {move goal up}
\todo {incorporate in goal - the second observation in class of workloads}
\todo{contention in rop is a factor - set this up first before discusing}
Our \textbf{goal} in this work is to accelerate raster-based inverse rendering applications by alleviating the atomic bottleneck at sub-core level\todo{sm level?}. 
To this end, we introduce \projname, a primitive that alleviates the \todo{accelerates atomics} LSU contention due to atomic operations in applications where a high number of threads aggregate common parameters atomically. 
The key idea of \projname is to provide efficient hardware support to find and aggregate common parameters computation at the sub-core level, to update within each warp update the same gradient parameter, to express part of the gradient summation to be performed at each SM core, and a part to be done in the ROP units such that are not kept starved from processing. 
The gradient parameter reduction work then be scheduled either in the SM core, or the ROP units, depending on the level of contention of hardware resources.   
Hence, we propose \textbf{(1)} A software approach that selects and schedules the computation of atomic reduction processing, either in the SM core or the L2 ROP units based on the level of contention of each hardware resource. This approach performs a reduction at the SM-core level using warp level primitives (such as\emph{\_\_shfl\_sync}) to access thread data from different warps and aggregate them using a FP unit. As each thread has to update several parameter of the primitive, this requires a check across warps to find the common address for each parameter. To alleviate this checks in doing reduction, the single primitive index for aggregation. 

A key challenge in this approach is determining the level of contention in the SM core and the L2 ROP partition, and managing while introducing minimal overhead at runtime. To address this, we introduce a hyperparameter which determines the number of summations to be performed in the SM core for doing reduction compared to the computation offloaded to the L2 ROP units. 

However, this approach requires hyperparameter tuning and a significant programming effort in implementing this solution. Additionally, the additional code introduced to do reduction at the sub-core level introduces additional control flow and compute latency overhead which could slow down the application.  
\textbf{(2)} In order to solve this, we propose \projname-HW solution, a HW mechanism that adaptively determines which parameters can be summed up at the SM level for doing reduction, and adaptively schedules the overall reduction computation to either the SM core or the L2 partition, based on the level of contention of these HW resources. \todo{approahc - go through how hw does it}

\todo{provide more references}
We evaluate our approach across recent widely used inverse rendering workloads. With our SW approach, we achieve a speedup of up to \todo{}$\times$ on the backward shader kernel alone, and up to \todo{}$times$ overall application speedup. With \projname-HW, we achieve a speedup of up to \todo{}$\times$ on the shader kernel, and an upto  $\times$ overall speedup. Our list of contributions are summarized as follows: 
\begin{itemize}
    \item We provide a detailed characterization of rasterization + shading based on a wide range of inverse rendering workloads
    \item Design our software approach to alleviate the bottleneck associated with reduction operations in computing the backward pass gradients.
    \item Design \projname-HW, a HW mechanism that adaptively chooses reduction operation based on the level of contention of resources at the ROP units and the SM core.

\end{itemize}








==> text_srcs_old/introduction_2.tex <==
Differentiable rendering leverages machine learning to solve several fundamental problems in computer graphics, such as scene reconstruction (deriving a representative model of a 3D scene)~\cite{nerf,dvgo,3dgs},
and inverse rendering~\cite{nvdiffrec, nvdiffrecmc} (infer properties of the 3D environment such as geometries of objects, color, and material properties) from a set of captured images of the scene.
These problems are central to several current and emerging applications, such as photogrammetry, 3D modeling and scanning, 3D model creation tools, game engines, and AR/VR applications. 
With differentiable rendering, these problems are formulated as a learning problem that can be solved by incorporating gradient-based optimization techniques. 

For example, neural radiance fields~\cite{nerf, dvgo, plenoxels, instantngp, mipnerf, mipnerf360, zipnerf} represent the scene by parameterizing the radiance information at each point in space using a neural network. It then computes a loss between a rendered image and the corresponding ground truth image, which is minimized using gradient descent. A differentiable renderer is used to compute the loss gradients with respect to these scene parameters~\cite{volume_rendering}.  
The use of learning based methods for these tasks demonstrated significant success in retrieving state-of-the-art quality scene representations, leading to huge interest in the computer graphics community. This success has led to several specialized frameworks and libraries for differentiable rendering~\cite{nvdiffrast,pytorch3d, mitsuba, drjit, difftaichi} as well as recent work~\cite{slang, slangd} proposing native support for differentiable rendering in GPUs as a first-class feature. 

% A 
Another widely-used scene representation method to encode visual information is to consider the scene as being composed of a large set of geometric \emph{primitives} in 3D space. These primitives could be triangles, spheres, rectangles, etc., with each primitive associated with color information. These primitives can be rendered on screen using a high-speed rasterization pipeline~\cite{opengl}. Several recent works~\cite{3dgs, pulsar, nvdiffrec, dmtet, flexicubes, adop} incorporate differentiable raster-based renderer in learning each primitives' parameters (position, color, etc.) on these aforementioned tasks.  
Among these methods, a recent transformative work, 3D gaussian splatting~\cite{3dgs}, has spurred tremendous interest in the computer graphics community~\cite{x}. It has demonstrated state-of-art capability in producing high-accuracy, high-quality scene reconstructions at a very high speeds, and has emerged a promising fundamental representation for 3D visual data. It represents the scene geometry with 3D gaussians as its primitives, and associates each gaussians with a view-direction dependent color. It uses an efficient tile-based rasterizer~\cite{adop, pulsar} over the 3D gaussians which are then colored to produce an image of the scene.  
The sheer level of successes of this method led to its adoption in Unreal Engine~\cite{unreal}, a mature 3D modelling application / game engine, where it is used to obtain a 3D model of the real-world.

% These primitives constitute the 3D scene. 
In this work, we consider raster-based differentiable rendering implementations for GPUs, referred to as \emph{backward shading} kernel.
The backward shading kernel takes as input the loss gradient w.r.t to the image and computes the gradient w.r.t the each primitive's parameters.
Each thread of the backward shader kernel is associated with one pixel. It computes and then accumulates the gradient contribution of each primitive w.r.t its pixel color.
This backward-pass of shader routine constitutes a significant bottleneck in the overall application, taking up as much as 30-70\%\todo{check} of the overall time (see section~\ref{sec:motivation_backward_runtime}). 
We observe this bottleneck is primarily caused by an overwhelming number of atomic operations launched during gradient accumulation step.
% . The atomic operations issued by the sub-cores are queued to the instruction queue leading to the LSU (Load-Store-Unit) that handles memory operations in the SM. 
% This causes high contention at the LSU. (Section~\ref{sec:motivation_shaderbwdimpl}).
% This high-number of atomic operations
This is a consequence of rendering highly detailed scene into a high resolution image. The number of atomic requests grows rapidly with image size (proportional to the number of pixels/quadratically with the resolution), linearly with number of primitives contributing to the color of a pixel, and linearly with the number of trainable parameters per primitive. In-effect, this overwhelmingly high number of atomic operations causes high contention at the LSU (Load-Store-Unit), which handles memory operations in the SM (see Section~\ref{sec:motivation_backward_runtime} and Section~\ref{sec:motivation_shaderbwdimpl} for details).

% Hence, each pixel is associated with a large number of primitives, and each primitive has many parameters.



Our \textbf{goal} in this work is to accelerate raster-based differentiable rendering applications by accelerating atomic operations that constitute a significant bottleneck in these applications. 
We make the following key observation from our analysis of the atomic operations in the backward pass of differentiable rendering workloads: threads in a warp typically update parameters of few distinct primitives. In fact, we find that the number of warps having all threads update the same primitive are up to 95\%. This leads to a large number of threads in a warp to add gradient updates to the same set of memory addresses via atomic requests. 
Prior approaches~\cite{lab, massiveatomics, acceleratingatomics} address bottlenecks due to atomic requests with SM-level reduction before sending them to the memory partition.  
This involves aggregating individual atomic requests produced by each thread on the L1/shared memory. However, aggregating atomic requests at the SM-level will not alleviate contention at the LSU, as atomic requests only arrive at L1/shared memory after it leaves the LSU. 
Hence, to this end, we introduce \projname, a primitive that accelerates the processing of atomic operations in applications where a high number of threads aggregate common parameters atomically. 
The key idea of \projname is to aggregate common parameters' reduction computation at the sub-core level, to update the same gradient parameter. We express part of the gradient summation to be performed at each sub-core, and a part to be done in the ROP units (in the memory subpartition, which perform atomic operation computation) such that are not kept starved from processing.
% The gradient parameter reduction work then be scheduled either in the sub-core, or the ROP units, depending on the level of contention of hardware resources.

We implement two versions of \projname:  \textbf{(1) \projname-SW}: A software approach that selects and schedules the computation of atomic reduction processing, either in the sub-core or the ROP units based on the level of contention of each hardware resource. At the sub-core level, we aggregates atomic requests for several parameters of each geometric primitive using warp-level instructions (such as\emph{\_\_shfl\_sync}) for doing reduction across threads. 
% However, this approach requires hyperparameter tuning and a significant programming effort in implementing this solution. Additionally, the additional code introduced to do reduction at the sub-core level introduces additional control flow and compute latency overhead which could slow down the application.  
\textbf{(2) \projname-HW}: The additional code introduced to do reduction at the sub-core level introduces additional control flow and compute latency overhead which could slow down the application in our SW implementation. In order to solve this, we propose \projname-HW solution, a HW mechanism that adaptively selects either the sub-core or ROP units for doing reduction based on resource availability. 
We modify the sub-core's instruction pipeline to process atomic reduction operations. As part of our design, we introduce a new, low-overhead execution unit at each sub-core. This module contains an FP unit to perform the reduction and sends the result to the LSU instruction queue. Our HW sub-core logic packs common atomic requests across different threads in a warp together into a single transaction. On issuing this transaction, \projname checks whether the LSU instruction queue is busy to issue requests to. If busy, \projname schedules the transaction to the reduction module to do the reduction.

We evaluate our approach across recent widely used differentiable rendering workloads. With our SW approach, we achieve a speedup of up to \todo{}$\times$ on the backward shader kernel alone, and up to \todo{}$\times$ overall application speedup. With \projname-HW, we achieve a speedup of up to \todo{}$\times$ on the shader kernel, and an up to  $\times$ overall speedup. Our list of contributions are summarized as follows: 
\begin{itemize}
    \item We provide a detailed characterization of rasterization + shading based on a wide range of differentiable rendering applications.
    \item Design \projname-SW, a SW approach that uses either using warp-level primitives to perform reduction computation at the sub-core level, or schedule the computation to the ROP units based on resource usage.
    \item Design \projname-HW, a HW mechanism that performs a efficient atomic reduction computation on utilizing the sub-core's as well as ROP's floating point units.
    \item We will provide an open-source, software-only implementation of \projname that can be used on real hardware to enable fast raster-based differentiable rendering.

\end{itemize}








==> text_srcs_old/introduction_3.tex <==
Differentiable rendering leverages machine learning to solve several fundamental problems in computer graphics, such as scene reconstruction (deriving a representative model of a 3D scene)~\cite{nerf,dvgo,3dgs},
and inverse rendering~\cite{nvdiffrec, nvdiffrecmc} (infer properties of the 3D environment such as geometries of objects, color, and material properties) from a set of captured images of the scene.
These problems are central to several current and emerging applications, such as photogrammetry, 3D modeling and scanning, 3D model creation tools, game engines, and AR/VR applications. 
With differentiable rendering, these problems are formulated as a learning problem that can be solved by incorporating gradient-based optimization techniques. 

For example, neural radiance fields~\cite{nerf, dvgo, plenoxels, instantngp, mipnerf, mipnerf360, zipnerf} represent the scene by parameterizing the radiance information at each point in space using a neural network. It then computes a loss between a rendered image and the corresponding ground truth image, which is minimized using gradient descent. A differentiable renderer is used to compute the loss gradients with respect to these scene parameters~\cite{volume_rendering}.  
The use of learning based methods for these tasks demonstrated significant success in retrieving state-of-the-art quality scene representations, leading to huge interest in the computer graphics community. This success has led to several specialized frameworks and libraries for differentiable rendering~\cite{nvdiffrast,pytorch3d, mitsuba, drjit, difftaichi} as well as recent work~\cite{slang, slangd} proposing native support for differentiable rendering in GPUs as a first-class feature. 

A widely-used scene representation method to encode visual information is to consider the scene as being composed of a large set of geometric \emph{primitives} in 3D space(i.e. triangles, spheres, rectangles). Each primitive is associated with color information. This raster-based differentiable rendering method is efficient as these primitives can be rendered on screen using a high-speed rasterization pipeline~\cite{opengl}. Several recent works~\cite{3dgs, pulsar, nvdiffrec, dmtet, flexicubes, adop} incorporate differentiable raster-based renderer in learning each primitives' parameters (position, color, etc.) on these aforementioned tasks.  
Among these methods, a recent transformative work, 3D gaussian splatting~\cite{3dgs}, has spurred tremendous interest in the computer graphics community~\cite{x}. It has demonstrated state-of-art capability in producing high-accuracy, high-quality scene reconstructions at a very high speeds, and has emerged a promising fundamental representation for 3D visual data. It represents the scene geometry with 3D gaussians as its primitives, and associates each gaussians with a view-direction dependent color. It uses an efficient tile-based rasterizer~\cite{adop, pulsar} over the 3D gaussians which are then colored to produce an image of the scene.  
The sheer level of successes of this method led to its adoption in Unreal Engine~\cite{unreal}, a mature 3D modelling application / game engine, where it is used to obtain a 3D model of the real-world.
Owing to the speed and quality advantages inherent in these methods, differentiable rendering on raster-based pipelines firmly establishes itself as a promising approach for the future.

To investigate the existing limitation of raster-based differentiable rendering methods and advance towards real-time differentiable rendering, we performed a comprehensive profiling on several important differentiable rendering workloads using state-of-the art raster-based methods. We discovered that the backward pass of shader routine constitutes a significant bottleneck, taking up as much as 30-70\%\todo{check} of the overall training time (see section~\ref{sec:motivation_backward_runtime}).
% Hence, in this work, we focus on these raster-based differentiable rendering implementations for GPUs, which constitute a family of widely methods for 3D scene reconstruction and inverse rendering tasks.
Our analysis of the raster-based rendering pipeline shows that this bottleneck is primarily caused by an overwhelming number of atomic operations that accumulates gradients for primitive parameters. During backward pass, each thread is associated to one pixel. It computes and then accumulates the parameter gradients for all primitives the pixel is associated with. As different pixels can be influenced by the same primitive, the gradient update for each primitive parameter are performed with atomic operations to avoid racing conditions across the threads. This leads to a high number of atomic operations being launched by each thread, since the color of each pixel is influenced by a set of primitives, and each primitive contains several parameters. These atomic operations cause high degree of contention at each sub-core's memory instruction queue and stalls the memory pipeline, leading to a slowdown(see Section~\ref{sec:motivation_shaderbwdimpl} for details).

% Hence, each pixel is associated with a large number of primitives, and each primitive has many parameters.

Our \textbf{goal} in this work is to accelerate raster-based differentiable rendering applications by accelerating the processing of atomic operations that constitute a bottleneck in these applications. One possible approach to alleviate the bottleneck due to atomic reduction operations is to offload some of the the atomic reduction computation locally to the SM. This is possible to do when several threads executing within the SM atomically update a same addresses. 
Our analysis of the nature of the atomic operations in the backward pass of differentiable rendering workloads does indicate that all threads within a warp typically update parameters of few distinct primitives. Moreover, we find that the number of warps having all threads update the same primitive are up to 95\% (see Section~\ref{sec:motivation_observations}). 
% This leads to a large number of threads within a warp to add gradient updates to the same set of memory addresses via atomic requests. 
Prior approaches~\cite{lab, massiveatomics, acceleratingatomics} address bottlenecks due to atomic requests with SM-level reduction before sending them to the memory partition.
This involves aggregating individual atomic requests produced by each thread at the L1/shared memory. However, the number of atomic operations issued by differentiable rendering workloads is so overwhelmingly high, that it causes contention at the SM's Load Store Unit (LSU, which handles memory instructions to/from the SM) itself. This leads to stalls at the sub-cores, which cannot be alleviated with reductions at L1/shared memory. 



In this work, we introduce \projname, a primitive that accelerates the processing of atomic operations in applications which \textbf{(i)} produce an overwhelmingly high number of atomic reduction operations during execution, and \textbf{(ii)} consisting of a large number of threads within each warp aggregating to a common parameter atomically.
The key idea of \projname is to \textbf{(i)} Aggregate common parameters' reduction computation at the sub-core level, to update the same gradient parameter, and \textbf{(ii)} Do part of the gradient summation operation at the sub-cores, and a part at the ROP units (in the memory subpartition, which performs atomic operation computation) to increase utilization of available computation units in doing reduction.
% The gradient parameter reduction work then be scheduled either in the sub-core, or the ROP units, depending on the level of contention of hardware resources.

We implement two versions of \projname:  \textbf{(1) \projname-SW}: A software approach that utilizes a tunable hyperparameter, which we refer to as the \textit{balancing threshold}, to perform opportunistic sub-core level atomic reduction. It dynamically detects the number of threads in a warp that actively participates in an atomic operation with common addresses. It performs warp-level aggregation when this number is larger than the balancing threshold. We implemented \projname-SW with existing warp-level programming primitives(such as\emph{\_\_shfl\_sync}) to enable atomic reduction at sub-core level, even when only a subset of warp threads actively participate in the reduction.
% However, this approach requires hyperparameter tuning and a significant programming effort in implementing this solution. Additionally, the additional code introduced to do reduction at the sub-core level introduces additional control flow and compute latency overhead which could slow down the application.  
\textbf{(2) \projname-HW}: The additional code introduced to do reduction at the sub-core level introduces additional control flow and compute latency overhead which could slow down the application in \projname-SW implementation. In order to solve this, we propose \projname-HW solution, a HW mechanism that adaptively selects either the sub-core or ROP units for doing reduction based on resource availability. 
We modify the sub-core's instruction pipeline to process atomic reduction operations. As part of \projname's design, we introduce a new, low-overhead execution unit at each sub-core. This module contains an FP unit to perform the reduction and sends the result to the LSU instruction queue. \projname-HW's sub-core logic packs common atomic requests across different threads in a warp together into a single transaction. On issuing this transaction, \projname checks whether the LSU instruction queue is busy to issue requests to. If busy, \projname schedules the transaction to the reduction module to do the reduction.

We evaluate \projname across recent widely used differentiable rendering applications (3D Gaussian Splatting~\cite{3dgs}, NVDIffRec~\cite{nvdiffrec}, Pulsar~\cite{pulsar, pytorch3d}) on different datasets (Section~\ref{sec:methodology}). With \projname-SW, we achieve a speedup of up to \todo{}$\times$ for the backward pass kernel, and up to \todo{}$\times$ overall application speedup. With \projname-HW, we achieve a speedup of up to \todo{}$\times$ on the shader kernel, and an up to  $\times$ overall speedup. Our list of contributions are summarized as follows: 
\begin{itemize}
    \item We provide a detailed characterization of rasterization + shading based on a wide range of differentiable rendering applications.
    \item Design \projname-SW, a SW approach that uses either using warp-level primitives to perform reduction computation at the sub-core level, or schedule the computation to the ROP units based on resource usage.
    \item Design \projname-HW, a HW mechanism that performs a efficient atomic reduction computation with maximum utilization of the sub-core's as well as ROP's floating point units.
    \item We will provide an open-source, software-only implementation of \projname that can be used on real hardware to enable fast raster-based differentiable rendering.

\end{itemize}








==> text_srcs_old/methodology.tex <==

\label{sec:methodology}

\textbf{Evaluation Platform.} 
We implement and evaluate \projname-SW on real hardware setups with an Intel Core i9 13900KF CPU (specifications shown in Table~\ref{tab:cpuconfig}) and the NVIDIA RTX4090 and RTX3060 GPUs. We model and evaluate \projname-HW using the GPGPU-Sim simulator~\cite{accelsim} with the RTX4090 and RTX3060 GPU configuration (shown in Table~\ref{tab:gpusim_4090} and Table~\ref{tab:gpusim_3060}). 

\begin{table}[h!]
  \centering
  \caption{CPU system configuration}
  \label{tab:cpuconfig}
  \begin{tabular}{|l|}
    \hline
    \hline
     \textbf{CPU} 3.6GHz Rocket-lake-like, OOO 4-wide dispatch window,\\ 128-entry ROB; 32 entry LSQ \\
    \hline
     \textbf{L1D + L1I Cache} 32KB, 4 way LRU, 1 cycle; 64 Byte line; \\ MSHR size: 10; stride prefetcher \\
    \hline
     \textbf{L2 Cache}  256KB, 8 way LRU, 4 cycle; 64 Byte line; \\ MSHR size: 10; stride prefetcher \\
    \hline
     \textbf{L3 Cache} 1MB, 16 way LRU, 20 cycle; 64 Byte line; \\ MSHR size: 64; stride prefetcher \\
    \hline
     \textbf{DRAM} 2-channel; 16-bank; open-row policy, 4GB DDR4\\
    \hline
  \end{tabular}

\end{table}


\begin{table}[h!]
 \centering
  \caption{Simulated GPU configuration - RTX 4090}
  \label{tab:gpusim_4090}
  \begin{tabular}{|l|}
    \hline
    \hline
     \textbf{SM Resources} 144 SMs, 32768 Registers, 32KB Shared memory,\\ 128KB L1D, 4 ways \\
    \hline
     \textbf{Shader core} 1.4GHz; 4 sub-cores per SM \\
    \hline
     \textbf{Memory Model} FCFS scheduling, 16 banks/channel\\
    \hline
     \textbf{DRAM} 2-channel; 16-bank; open-row policy, 24GB DDR4 \\
    \hline
  \end{tabular}
\end{table}


\begin{table}[h!]
 \centering
  \caption{Simulated GPU configuration - RTX 3060}
  \label{tab:gpusim_3060}
  \begin{tabular}{|l|}
    \hline
    \hline
     \textbf{SM Resources} 28 SMs, 32768 Registers, 32KB Shared memory,\\ 128KB L1D, 4 ways \\
    \hline
     \textbf{Shader core} 1.4GHz; 4 sub-cores per SM \\
    \hline
     \textbf{Memory Model} FCFS scheduling, 16 banks/channel\\
    \hline
     \textbf{DRAM} 2-channel; 16-bank; open-row policy, 12GB DDR4 \\
    \hline
  \end{tabular}
\end{table}





\textbf{Workloads.} We evaluate our approach using widely used applications that use differentiable rasterization for inverse rendering, which we describe here:

\begin{itemize}
    \item \textbf{\texttt{3DGS}}: 3D Gaussian Splatting~\cite{3dgs} is a recent work that represents the scene with a set of 3D gaussians. Each gaussian is associated with a view dependent radiance, and associated with a position and orientation in 3D space. 3D Gaussian Splatting is used to obtain high-quality 3D reconstruction of a scene captured with cameras overlooking the scene.  
    
    \item \textbf{\texttt{nvdrec}}: Nvdiffrec~\cite{nvdiffrec} is a large project that can be used for various tasks in inverse rendering (deriving scene properties from a set of captured images). For our evaluation, we use differentiable rendering to learn the parameters of specular cubemap texture on a mesh (which can be rasterized), from a set of images capturing the mesh. 
    
    \item \textbf{\texttt{pulsar}}: Pulsar~\cite{pulsar, pytorch3d} is a recent work for 3D scene reconstruction, that represents the scene with a set of spheres in 3D space. Pulsar incorporates an efficient sphere rasterizer implementation that is used to render the scene composed of spheres on screen. This implementation is incorporated into Pytorch3D~\cite{pytorch3d}, a widely used framework with for differentiable rendering. 

    % \item \textbf{\texttt{adop}}: ADOP~\cite{adop} uses pixel rasterization to 

\end{itemize}

We evaluate \projname using the datasets listed in Table~\ref{table:datasets}. 

\begin{table}[h!]
 \centering
  \caption{Workloads and datasets}
  \label{table:datasets}
  \begin{tabular}{|l|l|l|}
    \hline
     \multirow{2}{*}{\textbf{Workloads}}     & \textbf{Dataset}      & \textbf{Dataset} \\
                                             & \textbf{identifier}   & \textbf{name} \\
    \hline
    \multirow{5}{*}{\texttt{3DGS}} &  \texttt{T\&T} & Tanks and Temples~\cite{tandt}   \\
                                   &  \texttt{NS-T} & NerfSynthetic-Truck~\cite{nerf}       \\
                                   &  \texttt{NS-S} & NerfSynthetic-Ship~\cite{nerf}       \\
                                   &  \texttt{PR}   & Playroom~\cite{playroom}       \\
                                   &  \texttt{DR}   & DR. Johnson~\cite{drjohn}       \\
    \hline
    \multirow{2}{*}{\texttt{nvdrec}} &  \texttt{BOB} &  Keenan Crane 3D model repository~\cite{crane}   \\
                                    &  \texttt{SPOT} &  Keenan Crane 3D model repository~\cite{crane}   \\
                                   &  \texttt{NS-T}    & NerfSynthetic~\cite{nerf} - Truck      \\
                                   &  \texttt{NS-R}    & NerfSynthetic~\cite{nerf} - Ship       \\
    \hline
    \multirow{2}{*}{\texttt{pulsar}} &  \texttt{SSS}   & Synthetic Spheres   - Small  \\
                                     &  \texttt{SSL}   & Synthetic Spheres - Large       \\


    \hline

    % \multirow{2}{*}{\texttt{adop}} &  \texttt{T\&T}  & Tanks and Temples    \\
    %                                &  \texttt{NS}    & NerfSynthetic       \\
    % \hline

  \end{tabular}
\end{table}


\subsection{\projname Configurations}

We evaluate \projname on several configurations, which we describe in Table~\ref{tab:methodconfigurations}. \texttt{SW-B-X} and \texttt{SW-S-X} are the SW configurations that use butterfly reduction and serialized addition to do reduction respectively, with $X$ as the balancing hyperparameter. \texttt{SW-B} and \texttt{SW-S} are the software implementations with the best performing balancing hyperparameter for each workload.

\begin{table}[h!]
 \centering
  \caption{Workloads and datasets of our experiments}
  \label{tab:methodconfigurations}
  \begin{tabular}{|l|l|}
    \hline
     \textbf{Configuration}    & \textbf{Description} \\

    \hline
    \multirow{2}{*}{\texttt{SW-B-X}} &  SW approach with butterfly-reduction, \\                                      & with X as the balance threshold   \\
    \hline
    \multirow{2}{*}{\texttt{SW-S-X}} &  SW approach with serialized-reduction, \\                                      & with X as the balance threshold   \\
    \hline
    \texttt{SW-B} &  SW w/ butterfly-reduction, best case \\
    \hline
    \texttt{SW-S} &  SW w/ serialized-reduction, best case \\     

    \hline
    \texttt{\projname-HW} &  \projname HW implementation    \\             

    \hline

  \end{tabular}
\end{table}





==> text_srcs_old/motivation.tex <==
\subsection{Time Spent in Shader's Backward Pass}
\todo{change title: look at other papers "ineff. bwd pass"} 
\label{sec:motivation_backward_runtime}
% As described in Section~\ref{sec:bckg_diffrendering}, the forward pass of the raster-based rendering pipeline involves first rendering an image from a parameterized scene representation. A loss is then computed as the difference between the rendered image and the ground truth. On backpropagating this loss, we can find the gradient of the loss with respect to the scene parameters, enabling us to perform gradient based optimization on these scene parameters.

The backward pass of the shader kernel occupies a significant amount of time of the overall inverse rendering process. 
We conduct an experiment to find the percentage of time taken by the backward pass of the shader as a percentage of overall runtime for various inverse rendering applications (see Section~\ref{sec:methodology}) in Fig.~\ref{fig:backward_runtime}. We observe that up to \todo{} $60\%$  of the total runtime is spent on the backward shader kernel, showing that the backward shader kernel constitutes a significant bottleneck. 

% \todo{several small bars with lowest blue bar depicting bwd} 


\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/temp/perc_backward_kernel.png}
    \caption{Percentage of time spent on backward pass of the shader during training}
    \label{fig:backward_runtime}
\end{figure}



% \subsection{Atomic Reduction Bottleneck in the Backward Pass}

% \subsection{Implementation outline of the backward shader kernel}
% \label{sec:motivation_shaderbwdimpl}
% Here, we inspect the backward shader kernel in further detail. \todo{is this professional?}

Each thread of the kernel corresponds to a single pixel. Associated with each pixel is a list of geometric primitives which contributes to the pixel's color (see Section~\ref{sec:bckg_diffrendering}).
The thread receives this list of primitives as input and computes the gradients of the parameters' of each primitive with respect to the corresponding pixel gradient. 
% the gradient of a loss function with respect to parameters of scene primitives, from the gradient loss with respect to the pixel color channels.
\todo{write like this is general -  mimicked in different applications}
The implementation of the backward shader kernel has the general structure shown in Fig.~\ref{fig:atomicimplementation}. The program execution flow is as follows: each thread iterates through a list of its associated primitives. It then determines if \todo{it} is going to contribute a non-zero gradient to the current primitive (based on conditions $cond1, cond2, ..$). Each primitive is associated with several trainable parameters $x1, x2, x3, ...$. The thread then computes the gradient contribution of the primitive's parameters ($grad_t x1, grad_t x2, ...$). Finally, it performs an atomic add operation to accumulate it's gradient contributions to the primitive's parameters. 

There are several conditional branches that lead to divergence of threads during the execution of each thread. This typically lead to only a subset of the threads are going to perform an atomic operation.
\todo{refernce lines in the algorithm with line numebr, insert comments in the algorihtm
}
\begin{figure}[!htb]

 \colorbox[RGB]{239,240,241}{
     \begin{minipage}{.9\linewidth}
\begin{algorithmic}

\Function{BwdShaderKernel}{prims\_per\_thread}

\State $tid \gets thread\_idx$
\State $prims\_per\_thread \gets primitives[tid]$

\For{ $p : prims\_per\_thread$ }

\If{ \Call{cond1}{} }
    \State \textbf{continue;}
\EndIf

    \State ...    
\If{ \Call{cond2}{} }
    \State \textbf{continue;}
\EndIf
    \State ...    
    \State \Call{AtomicAdd}{$p.grad\_x1$,  $\nabla^{tid}_{x1} $}
    \State \Call{AtomicAdd}{$p.grad\_x2$,  $grad_t x2$}
    \State \Call{AtomicAdd}{$p.grad\_x3$,  $grad_t x3$}
    \State ...    

\EndFor

\EndFunction
\end{algorithmic}

\end{minipage}

}

\caption{Outline of the shader's backward pass \todo{better notation for per pixel gradient}} 
\label{fig:atomicimplementation}
\end{figure}


\todo{merge with previous, half this size, remove glue sentences. don't confuse fig. with algorithm}
\subsection{Volume of Atomic Operations Made, and Atomic Reduction Bottleneck}

As each thread of the shader's backward pass kernel corresponds to a single pixel of the rendered image, a high resolution image would fully occupy all the SM cores of the GPU.
% The outline of the implementation of the kernel's computation performed by each thread is shown in 
From algorithm~\ref{fig:atomicimplementation}, we see that each thread iterates through a number geometric primitives, and each loop iteration consists of updating several parameters of the corresponding primitive.  
This means that a massive number atomic operations are processed (in the order of a few 10s to 100s of millions each iteration). These atomic summation operations lead to: 
\textbf{(1)} Oversubscription of atomic requests to the LSU instruction queue at each sub-core. \textbf{(2)} Contention in processing of atomic requests at the ROP units. 
\todo{reference methodology}
To evaluate the effect of this, we perform an experiment that counts the percentage of stalls caused by contention of the LSU instruction queue \todo{not known} (where atomic instructions are sent to) and show the results in Fig.~\ref{fig:atomics_bottleneck}. We observe a large percentage of stalls at these locations.

%This leads to a significant bottleneck in executing atomic parameter reductions at the L2 level.
%Executing these requires a long latency, as processing atomic operations requires an acquire and release operation to be performed along with a floating point addition. 

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/temp/perc_atom_stalls.png}
    \caption{Percentage of stalls resulting from execution of atomic operations as a percentage of all stalls}
    \label{fig:atomics_bottleneck}
\end{figure}

% Throttling of the L1 load requests (where atomics requests are sent)
% This is because of there are only a few 100s of ROP units in the memory partitions that process these atomics requests ( Section~\ref{sec:bckg_atomicprocessing}).



We also see that the NVIDIA RTX 4090 GPU has a larger percentage of stalls in issuing instructions to the LSU queue when compared to NVIDIA RTX 3060.
This is because more recent GPUs possess a higher shader compute compared to ROP compute. 
For instance, an NVIDIA RTX 4090 GPU, which has 144 SM cores and 196 ROP units in the memory partition would see a larger bottleneck in processing atomics compared to RTX 3060 GPU which has 28 SM cores and 86 ROP units in its 12 memory partitions. \todo{see if this is good enough}
% GPUs that pack a large number SM compute cores compared to the ROP units lead to a bottleneck in processing atomic operations, as the shader-core computation component is diminished with respect to that computed at ROP. 





\subsection{Key Observations on Atomic Operation Processing \todo{more general}}
\label{sec:motivation_observations}
Based on our analysis of the backward shader kernel, we make the following key observations:

\subsubsection{Observation 1} \textbf{Large degree of common parameters performed by atomic updates by the threads of the warp.}
Each primitive affects a region of pixels on the screen, known as a "fragment" (Section~\ref{sec:bckg_diffrendering}). As a result, close-by pixels that belong to the same fragment update the same primitive.  
% Each thread of the backward shader kernel iterates through a list of geometric primitives and updates its parameters (from algorithm~\ref{fig:atomicimplementation}).
Fig.~\ref{fig:raster_locality_schematic} shows how adjacent/close by pixels fall onto the same fragment on rasterization.  We see that a single primitive rasterized onto a set of pixel leads to nearby by pixels being updated by the same primitive. 


\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.7\linewidth]{example-image}
    \caption{Close by threads update the parameters of the same primitives, on fragments produced by rasterization.}
    \label{fig:raster_locality_schematic}
\end{figure}

This implies that threads within a warp, which correspond to a local region of pixels, compute the gradient component of the same primitive. 
These gradient components are then atomically summed up across threads to produce the parameter's gradient.
We perform an experiment to find the distribution of the nubmer of threads in each active warp that atomically update the same primitive's parameters. Fig.~\ref{fig:atomics_locality} shows a histogram of the total number of distinct primitive whose parameters are updated by each warp  (at each loop iteration of Algorithm~\ref{fig:atomicimplementation}). We observe that a large portion of threads in each warp update the gradients of the same primitive.  

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/temp/distinct_warp_atom_prim.png}
    \caption{Number of distinct primitives across 32 threads in a warp. 1 distinct primitive implies that all active threads in the same warp share the same primitive value, thus their atomic updates will target the same memory address determined by this shared primitive.}
    \label{fig:atomics_locality}
\end{figure}


\subsubsection{Observation 2} 
\textbf{Few threads within a warp do atomic updates.}
% not issuing atomic requests for gradient update
From algorithm~\ref{fig:atomicimplementation}, we see that shader's backward pass has certain conditions ($cond1, cond2, ...$), that allow some threads to skip the current iteration of gradient updates. This implies that only a fraction of all threads send out atomic request within each warp.
Which thread participates in the atomic reduction is dynamically determined, based on the \todo{look into application to determine this-  criterion is app. dependent}
We measure the average number of 
Fig.~\ref{fig:atomics_unconvergent_warp_instructions}. We observe that a varying fraction of threads within a warp produce atomic updates to global memory. 

\begin{figure}[!htb]
\begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/temp/hist_active_warp_thd_3dgs_playroom.png}
    \caption{Experiment conducted on 3DGS Playroom}
    \label{fig:atomics_unconvergent_warp_instructions}
\end{subfigure}~
\begin{subfigure}{.49\textwidth}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/temp/hist_active_warp_thd_nvdiff_lego.png}
    \caption{Experiment conducted on NvDiff Lego.}
    \label{fig:atomics_unconvergent_warp_instructions}
\end{subfigure}

    \caption{Number of threads participating in atomic reduction.}
\end{figure}

Existing approaches can leverage observation 1 to aggregate the atomic gradients updates at the SM-level.

\todo{connection to motivate our appraohc}
\subsection{Existing Approaches that Use SM Level Reduction}

We can leverage observations 1 and 2 
A traditional approach

Existing CUDA libraries and software frameworks~\cite{warplvlredcuda, cccl} can leverage unique property 1 to do warp-level or block-level reductions in the SM core, and then send a single atomic add instruction with the computed sum. However, this requires all threads within a warp to be active, and an additional check to be performed for all addresses to be the same, which may not necessarily be the case. Prior HW approaches~\cite{dab,lab} can leverage the property that several atomics update the same address by doing an warp level reduction. However, as only a fraction of the threads are active, the additional control flow latency introduced in doing an SM-level reduction will lead to buildup of a bottleneck in the SM core. This results in the shift in the atomic bottleneck from the memory partition to SM. This may not be optimal, as the ROPs in memory partitions are now underutilized. Hence, to address this problem, our  approach appropriately distributes the reduction computation work between the SM and the core.









==> text_srcs_old/related_work.tex <==

To our knowledge, our work is the first that identifies and characterizes the fundamental bottleneck associated with atomics operation processing in graphics workloads. Prior works have looked into atomic operations in certain ML workloads


\textbf{Acceleration for inverse rendering techniques} 
Recent works ~\cite{neurex, instant3disca, gennerf, artist, mobilenerf} propose acceleration methods in HW to enable fast training of Neural Radiance fields~\cite{nerf,instantngp} models. These acceleration works focus on a second/orthogonal family of methods in inverse rendering (compared to raster-based rendering methods), in which the primary bottleneck lies in accessing the features associated with loading the scene parameters to render the scene. These works do not address the contention due to summation of gradient parameters by atomic operations, despite it constituting a close second-biggest bottleneck. Raster-based differentiable rendering pipelines follow a different algorithm for rendering an image, where the primary bottleneck is in atomic gradient aggregation.

\textbf{Processing atomic near the core in CPUs and GPUs}

Several works for CPU multiprocessors~\cite{lhrc, phi, aim} add additional buffers in the core that aggregate atomic add operations produced by the core without writing to memory. In implementing the same principle in GPUs, local atomic buffering~\cite{lab} performs global atomic floating point summations at the SM-level first to reduce serialization of processing of atomic operations at the ROP units. This approach, however, fails to clear the bottleneck in the contention in the LSU instruction queue seen when issuing the atomic operations from sub-core to the LSU. Our approach handles the reduction at the sub-core level, reducing the traffic in the instruction queue that sends memory instructions to the SM's LSU. 

Deterministic atomic buffering~\cite{dab} is another approach that introduces SM-level and sub-core level buffers which buffer the  atomic requests as they occur in program order. The main motivation for doing this operations is to maintain the determinism in order of atomic execution, and leads to a slowdown when compared to relaxing this criterion. 

\textbf{Work on accelerating atomic operations}
\todo{several works here - need to carefully classify them. but they are less relevant}

GPUs use a simple software-driven cache coherence protocol without o
Prior work in trying to accelerating atomic operations on GPU architectures falls into two categories: one that switches the GPU memory consistency model into a weaker one, or latering the GPU's cache coherence protocol  ~\cite{gpucachecoherence, acceleratingatomics, massiveatomics}


\textbf{Changes to Memory consistency model }
The GPU memory model follows the partial store order (PSO) across several threads, in which the order of stores is not guaranteed to be relaxed~\cite{ptxconsistency}. A barrier / synchronization routine is used to control the order of store operations.


\cite{denovo,ccache,coup}

In contrast to this, atomic operations are guaranteed to be performed as indivisible operation across threads, in that the loads from and stores to the memory location of each thread have no race conditions between them. Several SW managed~\cite{} and HW managed~\cite{} memory consistency models have been proposed recent works, which can affect the implementation and performance characteristics of atomic operations. 




\textbf{Software approaches in doing warp level reduciton}
Frameworks such as NVIDIA's CUB / CCCL~\cite{cccl, cub, warpredblog} library provide several functions for doing reudciotn at a warp level using a reduction tree. Using these approaches out of the box, however, leads to a slowdown because each of these warp level reductions introduce a significant amount of instructions and control flow. Each iteration of the thread accumulates gradients of several parameters each time, and using a seperate reduction tree for each accumulatio leads to significant overhead (we show this in Section~\ref{sec:results}).


\textbf{Atomic operation bottleneck in ML workloads}
FuseGNN, BSSYNC and graph applications~\cite{fusegnn, bssync, lab} demonstrate a similar bottleenck in commmitting atomic operatiosns





    
% \textbf{Generalized faster training models} 
% Several accelerators for deep elarning training acceleration have been proposed to deal with the total amount of atomic operations 



==> text_srcs_old/results.tex <==


\subsection{Performance analysis}


\subsubsection{Speedup Analysis in SW}
Fig.~\ref{fig:end_to_end_speedup} shows the end-to-end speedup obtained for differentiable rendering applications described in Section~\ref{sec:methodology}, on using the SW configuration that gives us the best (among Table ~\ref{tab:methodconfigurations}). We observe that \projname-SW is able to provide a speedup of up to $3.40\times$, and on average $3.4\times$. This speedup is obtained on alleviating the the atomic contention in the backward shader kernel alone. 

\begin{figure}[!htb]
    \centering
    \includegraphics[width=.9\linewidth]{figs/temp/sw_real_speedup.png}
    \caption{Normalized end-to-end speedup on RTX 4090 and RTX 3060.}
    \label{fig:end_to_end_speedup}
\end{figure}

In Fig.~\ref{fig:kernel_speedup}, we depict the normalized speedup obtained on the backward shader kernel alone.
Fig.~\ref{fig:kernel_speedup_4090} and ~\ref{fig:kernel_speedup_3060} shows the speedup obtained on the backward pass of the shader kernel, on an RTX 3060 GPU and RTX 4090 GPU respectively. We observe a speedup of up to $5.7\times$ over baseline that uses butterfly reduction (\texttt{SW-B}). We also observe a higher level of speedup on the RTX 4090, compared to RTX 3060. This is because the atomic bottleneck becomes more pronounced on the RTX 4090 when compared to the compute (containing 144 SMs and 196 ROP units, when compared to just 28 SMs and 48 ROPs in the 3060). 
We observe only a slight speedup on the \texttt{nvdifrec} workload. This is because our SW approach introduces additional overhead due as a result of doing extra instructions in computing the reduction.

\begin{figure}[!htb]
\begin{subfigure}{0.49\textwidth}
    \centering
    \includegraphics[width=.9\linewidth]{figs/temp/sw_speedup_4090.png}
    \caption{Normalized kernel speedup on RTX 3060}
    \label{fig:kernel_speedup_4090}
\end{subfigure}

\begin{subfigure}{0.49\textwidth}
    \centering
    \includegraphics[width=.9\linewidth]{figs/temp/sw_speedup_3060.png}
    \caption{Normalized kernel speedup on RTX 3060}
    \label{fig:kernel_speedup_3060}
\end{subfigure}

    \caption{Normalized kernel speedup on different models and workloads.}
    \label{fig:kernel_speedup}

\end{figure}


% \begin{figure}[!htb]
%     \centering
%     \begin{subfigure}{0.235\textwidth}
%     \includegraphics[width=\linewidth]{figs/temp/sw_speedup_4090_3dgs_nvdiff.png}
%     \caption{RTX 4090.}
%     \label{fig:atomics_unconvergent_warp_instructions}
%     \end{subfigure}
%     ~\begin{subfigure}{0.235\textwidth}
%     \includegraphics[width=\linewidth]{figs/temp/sw_speedup_3060_3dgs_nvdiff.png}
%     \caption{RTX 3060.}
%     \label{fig:atomics_unconvergent_warp_instructions}
%     \end{subfigure}

%     \caption{Normalized speedup on different models and workloads}
% \end{figure}

\subsubsection{Speedup analysis on HW architecture}
Fig.~\ref{fig:hw_speedup_3dgs} and \ref{fig:hw_speedup_nvdiff} shows the speedup obtained on the backward kernel on using our proposed hardware architecture \texttt{\projname-HW}. We observe an average speedup of $5\times$ on using the hardware approach. We see that \texttt{\projname-HW} performs better than the SW approach, as it eliminates the control flow overehead introduced by the programmer in the software approach, and does not require any additional tuning of hyperparameters.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/temp/hw_3dgs_playroom.png}
    \caption{Normalized speedup on hardware simulator that emulates RTX 4090 and RTX 3060 on 3DGS Playroom with SM reduction and our SCAR-HW.}
    \label{fig:hw_speedup_3dgs}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/temp/hw_nvdiff_bob.png}
    \caption{Normalized speedup on hardware on NVDIff Bob.}
    \label{fig:hw_speedup_nvdiff}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/temp/hw_nvdiff_lego.png}
    \caption{Normalized speedup on hardware simulator that emulates RTX 4090 and RTX 3060 on NvDiff Lego.}
    \label{fig:hw_speedup_nvdiff}
\end{figure}


\subsection{SW bottleneck analysis}

\subsubsection{Varying the balancing threshold parameter}
Fig.~\ref{fig:balance_factor_3060_3dgs} and ~\ref{fig:balance_factor_4090_3dgs} show the end-to-end speedup obtained on varying the balancing threshold parameter on all our workloads for the 3D gaussian splatting workload on RTX 3060 and RTX 4090 respectively. Fig.~\ref{fig:balance_factor_3060_nvdr} and \ref{fig:balance_factor_4090_nvdr} shows the speedup obtained on varying the balance parameter on the \texttt{nvdifrec} workload. We observe that we achieve the highest level of speedup when the balancing threshold parameter is set to a parameter in-between the extremes. This shows that setting $0$ or $32$ as the balancing threshold leads to a bottleneck developed in subcore or ROP units respectively.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/temp/sw_balance_factor_4090_3DGS.png}
    \caption{Normalized speedup with varying balance factor $b$ on 3DGS with RTX 4090.}
    \label{fig:balance_factor_4090_3dgs}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/temp/sw_balance_factor_3060_3DGS.png}
    \caption{Normalized speedup with varying balance factor $b$ on 3DGS with RTX 3060.}
    \label{fig:balance_factor_3060_3dgs}
\end{figure}


\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/temp/sw_balance_factor_4090_nvdiff.png}
    \caption{Normalized speedup with varying balance factor $b$ on NvDiff with RTX 4090.}
    \label{fig:balance_factor_4090_nvdr}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/temp/sw_balance_factor_3060_nvdiff.png}
    \caption{Normalized speedup with varying balance factor $b$ on NvDiff with RTX 3060.}
    \label{fig:balance_factor_3060_nvdr}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/temp/sw_balance_factor_4090_pulsar.png}
    \caption{Normalized speedup with varying balance factor $b$ on Pulsar with RTX 4090.}
    \label{fig:balance_factor_3060_nvdr}
\end{figure}





\subsubsection{Instruction Count vs atomic ops count on varying the Balancing Threshold}

In order to determine the impact of changing the balancing parameter on ROP unit contention vs sub-core computation bottleneck, we perform an experiment to measure the number of atomic instructions issued vs instruction count normalized to the baseline. These results are depicted in Fig.~\ref{fig:instruction_count} for various workload configurations. We observe that on increasing the balancing threshold parameter, the number of instructions to be executed by the sub-core increases, which contributes to the bottleneck compute bottleneck in the SM. Concurrently, the number of atomic operation requests decreases, clearing up the bottleneck caused due to atomic operation contention. 


\begin{figure}[!htb]
    \centering
    \begin{subfigure}{0.235\textwidth}
    \includegraphics[width=\linewidth]{figs/temp/insn_red_3DGS_playroom_4090_SWB.png}
    \caption{SW-B Playroom}

        \end{subfigure}
    \begin{subfigure}{0.235\textwidth}
    \includegraphics[width=\linewidth]{figs/temp/insn_red_3DGS_playroom_4090_SWS.png}
    \caption{SW-S Playroom}

        \end{subfigure}

    \begin{subfigure}{0.235\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/temp/insn_red_3DGS_lego_4090_SWS.png}
    \caption{SW-S Lego}

        \end{subfigure}~
    \begin{subfigure}{0.235\textwidth}
    \includegraphics[width=\linewidth]{figs/temp/insn_red_3DGS_lego_4090_SWB.png}
    \caption{SW-B  Lego}

        \end{subfigure}    
   
    \caption{Executed instruction count and number of atomic operations in relation to the balance factor on {3DGS} with RTX 4090.}
    \label{fig:instruction_count}

\end{figure}


\subsection{Grouping several parameter updates of several primitives}
% Each thread updates several parameters corresponding to the same geometric primitive in each iteration, as seen in Alg.~\ref{fig:atomicimplementation}. This involves sending several atomic requests to the hardware (one for each parameter), requiring several acquire and release operations for each atomic update. In doing warp level reduction in Algorithms ~\ref{alg:butterfly} and \ref{alg:redserial}, we leverage the fact that each thread updates the parameters of a single primitive each iteration and group the reduction computation over all parameters in a single for loop. 

In Fig.~\ref{fig:wwo_prim_speedup}, we compare the runtime seen in the shader's backward kernel on updating all the parameters of a single primitive in a loop as opposed to calling the reduction functions ~\ref{alg:butterfly} and \ref{alg:redserial} once for every parameter.
We find a significant performance increase (of up to 4X) on updating evaluating the reduction operation on all parameters in a loop. This is because updating each parameter with a separate reduction routine produces several instructions by the compiler. The number of instructions executed is depicted in Fig.~\ref{fig:wwo_prim_executed_instructions}. We see that calling individual reduction function calls requires a significantly more instructions to be executed.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/temp/w_wo_prim_SWS_speedup_4090.png}
    \caption{Normalized speedup with and without primitive on various 3DGS scenes with RTX 4090.}
    \label{fig:wwo_prim_speedup}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/temp/w_wo_prim_SWS_einsn_4090.png}
    \caption{Number of executed instructions with and without primitive on various 3DGS scenes with RTX 4090.}
    \label{fig:wwo_prim_executed_instructions}
\end{figure}


\subsection{Energy analysis}
\label{sec:energy_analysis}

\projname requires fewer memory I/O requires (atomic requests) to be issued from the via queue to the memory sub-partition. As each memory issue through the interconnect requires consumes a significant amount energy (compared to the computation, which is equivalent in our case), \projname-HW is able to save energy significantly in this regard.
Fig.~\ref{fig:interconnect_traffic} shows the interconnect traffic change in using \projname in various workload - dataset configurations measured on NVIDIA RTX 4090, in which we observe a reduction in the interconnect traffic. The corresponding overall energy consumed is visualized in Fig.~\ref{fig:energy_consumed}. We observe that \projname delivers on average $\times$ energy savings.

\begin{figure}[!htb]
\begin{subfigure}{0.49\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{figs/temp/sm_l2_traffic_red_4090.png}
    \caption{Normalized reduction in total SM $\rightarrow$ L2 interconnect traffic in backward kernels on RTX 4090.}
    \label{fig:interconnect_traffic}
\end{subfigure}

% \begin{subfigure}{0.49\textwidth}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/temp/}
%     \caption{Normalized reduction in energy consumed by the backward shader kernel.}
%     \label{fig:energy_consumed}
% \end{subfigure}

\caption{Analysis of energy consumed}

\end{figure}






